PAPAL: A Provable PArticle-based Primal-Dual ALgorithm for Mixed Nash Equilibrium

We consider the non-convex non-concave objective function in two-player zero-sum continuous games. The existence of pure Nash equilibrium requires stringent conditions, posing a major challenge for this problem. To circumvent this difficulty, we examine the problem of identifying a mixed Nash equilibrium, where strategies are randomized and characterized by probability distributions over continuous domains. To this end, we propose PArticle-based Primal-dual ALgorithm (PAPAL) tailored for a weakly entropy-regularized min-max optimization over probability distributions. This algorithm employs the stochastic movements of particles to represent the updates of random strategies for the $\epsilon$-mixed Nash equilibrium. We offer a comprehensive convergence analysis of the proposed algorithm, demonstrating its effectiveness. In contrast to prior research that attempted to update particle importance without movements, PAPAL is the first implementable particle-based algorithm accompanied by non-asymptotic quantitative convergence results, running time, and sample complexity guarantees. Our framework contributes novel insights into the particle-based algorithms for continuous min-max optimization in the general non-convex non-concave setting.

==> parts/backup.tex <==
i.e. for all $(x_0^\top, y_0^\top), (x_1^\top, y_1^\top)$
    $$|f(x_0,y_0)-f(x_1,y_1)|\leq L_0\begin{Vmatrix}
    \begin{bmatrix}
        x_0-x_1\\
        y_0-y_1
    \end{bmatrix}
    \end{Vmatrix}.$$

    i.e. for all $(x_0^\top, y_0^\top)$, $(x_1^\top, y_1^\top)$
    $$
    \|\nabla f(x_0,y_0)-\nabla f(x_1,y_1)\|\leq L_1\begin{Vmatrix}
    \begin{bmatrix}
        x_0-x_1\\
        y_0-y_1
    \end{bmatrix}
    \end{Vmatrix}.
    $$

i.e. for all $(x_0^\top, y_0^\top)$, $(x_1^\top, y_1^\top)$
    $$
    \left\|\nabla^2 f(x_0,y_0)-\nabla^2 f(x_1,y_1)\right\|\leq L_2\begin{Vmatrix}
    \begin{bmatrix}
        x_0-x_1\\
        y_0-y_1
    \end{bmatrix}
    \end{Vmatrix}.
    $$




Unfortunately, for general min-max problems, such as non-convex non-concave case, even the existence of such a pair is highly non-trivial. It is necessary to find other possible definitions for the equilibria whose theoretical properties can be guaranteed. \citet{evtushenko1974some} raise the ``local optima'' by extending the Nash equilibria definition: when there exists a neighborhood such that $(x,y)$ is a Nash equilibria, then it is a ``local minimax point''. 
\citet{fiez2019convergence,jin2020local} have shown that the definition in \citep{evtushenko1974some} is ill-behaved due to the arbitrariness of the neighborhood, which is not ``local'' conceptually.
\citet{fiez2019convergence} propose \emph{Differential Stackelberg Equilibrium} which restrict the behavior Hessian matrix.
\citet{daskalakis2018limit,adolphs2019local,mazumdar2020gradient} studies the properties of $(\epsilon,\delta)$-local min-max points, which restrict the neighborhood to be a ball. 
\citet{jin2020local} highlighted the robustness of $(\epsilon,\delta)$-local min-max points and discussed the first-order and the second-order implications. Most of these work attempts to solve the general min-max problem in the sense of local equilibrium with variants of assumptions and restrictions. However, given the empirical implications, it is quite important to provide the global convergence guarantees without convexity/concavity from the theoretical view.



    \begin{algorithm}
\caption{Primal Dual algorithm for MNE} \label{alg:algorithm0}
\hspace*{0.02in} {\bf Input:} 
initial density $p_0(x)$ and $q_0(y)$, number of iterations $T$, outer-loop learning rates $\{\eta_t\}_{t=1}^T$ and $\{\tau_t\}_{t=1}^T$,  outer-loop hyper-parameters $\{\mu_t\}_{t=1}^T$; 
\hspace*{0.02in} 

{\bf Output:} estimated equilibrium   
$(X_T, Y_T)$

\begin{algorithmic} 
\STATE Initialize $X_0\sim p_0(x),\ Y_0\sim q_0(y)$

\FOR{$t=0$ to $T$}
    \STATE Solve $Y_t$ with  Eq.~\eqref{minimizer-q} 
    \STATE Solve $X_t$ with  Eq.~\eqref{minimizer-p}

\ENDFOR 

\end{algorithmic}
\end{algorithm}

\begin{theorem}\label{out-layer-thm}
    We set
    \begin{align}
        \gamma_t\mu_t&=\gamma_{t-1},\label{out-layer-1}\\
        \gamma_t\tau_t&\leq \gamma_{t-1}(\tau_{t-1}+\lambda_2),\label{out-layer-2}\\
        \gamma_t\eta_t&\leq\gamma_{t-1}(\eta_{t-1}+\lambda_2),\label{out-layer-3}\\
        \tau_t\eta_{t-1}&\geq\mu_t,\label{out-layer-4}
    \end{align}
    and assume that subproblem error bounds in each step-$t$ satisfy
    \begin{align}
        \mathrm{KL}(p_t\|p_t^*)&\leq\delta_{t,1}(p),\, \mathrm{KL}(q_t\|q_t^*)\leq\delta_{t,1}(q),\label{out-layer-5}\\
        \left|\mathbb{E}_p[\log(p_t/p_t^*)]\right|\leq\delta_{t,2}(p),\, &\left|\mathbb{E}_q[\log(q_t/q_t^*)]\right|\leq\delta_{t,2}(q),\, \, \, \, \forall\, p\in\mathcal{P}_2(\mathcal{X}),\, q\in\mathcal{P}_2(\mathcal{Y}),\label{out-layer-6}
    \end{align}
    for any $t\geq 1$, then
    \begin{align}\label{out-layer-result1}
        \sum_{t=1}^k\gamma_t Q(w_t,w)\leq&\gamma_1\eta_1\mathrm{KL}(p\|p_0)-\gamma_k(\eta_k+\lambda_2)\mathrm{KL}(p\|p_k)+\gamma_1\tau_1\mathrm{KL}(q\|q_0)\notag
        \\
        &-\gamma_k\left(\tau_k+\lambda_2-\frac{1}{4\eta_k}\right)\mathrm{KL}(q\|q_k)+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]+(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\},
    \end{align}
    for any $\epsilon>0$. Moreover, we have
    \begin{align}
        \gamma_k\left(\tau_k+\lambda_2-\frac{1}{4\eta_k}\right)\mathrm{KL}(q\|q_k)\leq&\gamma_1\eta_1\mathrm{KL}(p\|p_0)+\gamma_1\tau_1\mathrm{KL}(q\|q_0)+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]\notag
        \\
        &\, \, \, \, \, \, +(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\},\label{out-layer-result2}
        \\
        \gamma_k\left(\eta_k-\frac{1}{4(\tau_k+\lambda_2)}\right)\mathrm{KL}(p_k\|p_{k-1})\leq&\gamma_1\eta_1\mathrm{KL}(p\|p_0)+\gamma_1\tau_1\mathrm{KL}(q\|q_0)+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]\notag
        \\
        &\, \, \, \, \, \, +(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\},\label{out-layer-result3}
    \end{align}
\end{theorem}
\begin{proof}
    We conclude the following equalities when Lemma \ref{lemma:subproblem-optimal} applied to Eq.~\eqref{subproblem:q} and Eq.~\eqref{subproblem:p}
    \begin{align}
        &\int(\phi_t(y)+\lambda_1\|y\|^{2+\delta})(q_t^*-q)(y)dy+\lambda_2 \cE(q_t^*)-\lambda_2 \cE(q)=\tau_t[\text{KL}(q||q_{t-1}^*)-\text{KL}(q_t^*||q_{t-1}^*)]-(\tau_t+\lambda_2)\text{KL}(q||q_t^*),\label{optimal-y}
        \\
        &\int(\psi_t(x)+\lambda_1\|x\|^{2+\delta})(p_t^*-p)(x)dx+\lambda_2 \cE(p_t^*)-\lambda_2 \cE(p)=\eta_t[\text{KL}(p||p_{t-1}^*)-\text{KL}(p_t^*||p_{t-1}^*)]-(\eta_t+\lambda_2)\text{KL}(p||p_t^*).\label{optimal-x}
    \end{align}
    Denoting $\tilde{\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{p_{t-1}}[f(x,y)]+\mu_t\mathbb{E}_{p_{t-2}}[f(x,y)],\, \tilde{\psi}_t(x)=\mathbb{E}_{q_t}[f(x,y)]$ and  subtracting \eqref{optimal-y} and the equality derived from applying $q=q_t$ to \eqref{optimal-y} with \eqref{out-layer-5} and \eqref{out-layer-6}, we obtain
    \begin{align}
        &\int(\phi_t(y)+\lambda_1\|y\|^{2+\delta})(q_t-q)(y)dy+\lambda_2 \cE(q_t)-\lambda_2 \cE(q)\notag
        \\
        =&\int(\phi_t(y)+\lambda_1\|y\|^{2+\delta})[q_t^*-q-(q_t^*-q_t)](y)dy+\lambda_2(\cE(q_t^*)-\cE(q))-\lambda_2(\cE(q_t^*)-\cE(q_t))\notag
        \\
        =&\tau_t[\mathrm{KL}(q\|q_{t-1}^*)-\mathrm{KL}(q_t^*\|q_{t-1}^*)-(\mathrm{KL}(q_t\|q_{t-1}^*)-\mathrm{KL}(q_t^*\|q_{t-1}^*))]-(\tau_t+\lambda_2)[\mathrm{KL}(q\|q_t^*)-\mathrm{KL}(q_t\|q_t^*)]\notag
        \\
        =&\tau_t[\mathrm{KL}(q\|q_{t-1})-\mathrm{KL}(q_t\|q_{t-1})]-(\tau_t+\lambda_2)\mathrm{KL}(q\|q_t)+(\tau_t+\lambda_2)(\mathrm{KL}(q_t\|q_t^*)-\mathbb{E}_{q}[\log(q_t/q_t^*)])\notag
        \\
        &+\tau_t\{\mathbb{E}_{q}[\log(q_{t-1}/q_{t-1}^*)]-\mathbb{E}_{q_t}[\log(q_{t-1}/q_{t-1}^*)]\}
        \notag
        \\
        \leq&\tau_t[\mathrm{KL}(q\|q_{t-1})-\mathrm{KL}(q_t\|q_{t-1})]-(\tau_t+\lambda_2)\mathrm{KL}(q\|q_t)+(\tau_t+\lambda_2)(\delta_{t,1}(q)+\delta_{t,2}(q))+2\tau_t\delta_{t-1,2}(q),
    \end{align}
    as similar as above, we can also obtain
    \begin{align}
        &\int(\psi_t(x)+\lambda_1\|x\|^{2+\delta})(p_t-p)(x)dx+\lambda_2 \cE(p_t)-\lambda_2 \cE(p)\notag
        \\
        \leq&\eta_t[\mathrm{KL}(p\|p_{t-1})-\mathrm{KL}(p_t\|p_{t-1})]-(\eta_t+\lambda_2)\mathrm{KL}(p\|p_t)+(\eta_t+\lambda_2)(\delta_{t,1}(p)+\delta_{t,2}(p))+2\eta_t\delta_{t-1,2}(p).
    \end{align}
    Using the boundness of $f$, we have for any density function $q$ and $p$,
    \begin{align}
        \left|\int (p_t-\hat{p}_t)(x)f(x,y)q(y)dxdy\right|\leq\epsilon,\, \, \, \, 
        \left|\int (q_t-\hat{q}_t)(y)f(x,y)p(x)dxdy\right|\leq\epsilon,\notag
    \end{align}
    by adjusting the number of sampling points on $\hat{p}_t$ and $\hat{q}_t$. Therefore, summing up these equilities above and using the definition of the Max-Min gap function $Q$, we have
    \begin{align}
        &Q(w_t,w)+\iint[(p_t-p_{t-1})-\mu_t(p_{t-1}-p_{t-2})](x)f(x,y)(q_t-q)(y)dxdy\notag
        \\
        =&\int(\tilde{\phi}_t-\phi_t)(y)(q_t-q)(y)dy+\int(\phi_t(y)+\lambda_1\|y\|^{2+\delta})(q_t-q)(y)dy+\lambda_2 \cE(q_t)-\lambda_2 \cE(q)\notag
        \\
        &+\int(\tilde{\psi}_t-\psi_t)(x)(p_t-p)(x)dx+\int(\psi_t(x)+\lambda_1\|x\|^{2+\delta})(p_t-p)(x)dx+\lambda_2 \cE(p_t)-\lambda_2 \cE(p)\notag
        \\
        \leq&4(1+\mu_t)\epsilon+\tau_t[\mathrm{KL}(q\|q_{t-1})-\mathrm{KL}(q_t\|q_{t-1})]-(\tau_t+\lambda_2)\mathrm{KL}(q\|q_t)+\eta_t[\mathrm{KL}(p\|p_{t-1})-\mathrm{KL}(p_t\|p_{t-1})]\notag
        \\
        &-(\eta_t+\lambda_2)\mathrm{KL}(p\|p_t)+(\tau_t+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]+2\tau_t\delta_{t-1,2}(q)+(\eta_t+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]+2\eta_t\delta_{t-1,2}(p).
    \end{align}
    Noting that
    \begin{align}
        &\iint[(p_t-p_{t-1})-\mu_t(p_{t-1}-p_{t-2})](x)f(x,y)(q_t-q)(y)dxdy\notag
        \\
        =&\iint(p_t-p_{t-1})(x)f(x,y)(q_t-q)(y)dxdy-\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q)(y)dxdy\notag
        \\
        &+\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q_{t})(y)dxdy.
    \end{align}
    We have the estimation of the linear combination of $Q$ by summing up the resulting equalities which follow from combining the above two relations and multiplying both sides by $\gamma_t\geq 0$,
    \begin{align}
        \sum_{t=1}^k\gamma_t Q(w_t,w)\leq&\sum_{t=1}^k\gamma_t[\eta_t \mathrm{KL}(p\|p_{t-1})-(\eta_t+\lambda_2)\mathrm{KL}(p\|p_t)]+\sum_{t=1}^k\gamma_t[\tau_t \mathrm{KL}(q\|q_{t-1})-(\tau_t+\lambda_2) \mathrm{KL}(q\|q_t)]\notag
        \\
        &+\sum_{t=1}^k\gamma_t\left[\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q)(y)dxdy\right.\notag
        \\
        &\left.\, \, \, \, \, \, -\iint(p_t-p_{t-1})(x)f(x,y)(q_t-q)(y)dxdy\right]+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &-\sum_{t=1}^k\gamma_t\left[\tau_t \mathrm{KL}(q_t\|q_{t-1})+\eta_t \mathrm{KL}(p_t\|p_{t-1})+\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q_{t})(y)dxdy\right]\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]+(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\}.
    \end{align}
    The above equality, in view of \eqref{out-layer-1}-\eqref{out-layer-3} and the fact that $p_0=p_{-1}$ and $q_0=q_{-1}$, then implies that
    \begin{align}\label{main-estimate}
        \sum_{t=1}^k\gamma_t Q(w_t,w)\leq& \gamma_1\eta_1 \mathrm{KL}(p\|p_0)-\gamma_k(\eta_k+\lambda_2)\mathrm{KL}(p\|p_k)+\gamma_1\tau_1 \mathrm{KL}(q\|q_0)-\gamma_k(\tau_k+\lambda_2) \mathrm{KL}(q\|q_k)\notag
        \\
        &-\sum_{t=1}^k \gamma_t\left[\tau_t \mathrm{KL}(q_t\|q_{t-1})+\eta_t \mathrm{KL}(p_t\|p_{t-1})+\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q_{t})(y)dxdy\right]\notag
        \\
        &-\gamma_k\iint(p_k-p_{k-1})(x)f(x,y)(q_k-q)(y)dxdy+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]+(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\}.
    \end{align}
    Also note that by \eqref{out-layer-1} and \eqref{out-layer-4}, we have
    \begin{align}\label{part-estimate}
        &-\sum_{t=1}^k \gamma_t\left[\tau_t \mathrm{KL}(q_t\|q_{t-1})+\eta_t \mathrm{KL}(p_t\|p_{t-1})+\mu_t\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q_{t})(y)dxdy\right]\notag
        \\
        \leq&-\sum_{t=2}^k\left[\gamma_t\tau_t\mathrm{KL}(q_t\|q_{t-1})+\gamma_{t-1}\eta_{t-1}\mathrm{KL}(p_{t-1}\|p_{t-2})-\gamma_t\mu_t\|p_{t-1}-p_{t-2}\|_{TV}\|q_{t-1}-q_{t}\|_{L^1}\right]\notag
        \\
        &-\gamma_k\eta_k\mathrm{KL}(p_k\|p_{k-1})\notag
        \\
        \leq&-\gamma_k\eta_k\mathrm{KL}(p_k\|p_{k-1}),
    \end{align}
    where the first inequality is derived from Pinsker's inequality $\|p_{t-1}-p_{t-2}\|_{TV}\leq\sqrt{\mathrm{KL}(p_{t-1}\|p_{t-2})/2}$, $\|q_{t-1}-q_{t}\|_{L^1}\leq\sqrt{2\mathrm{KL}(q_t\|q_{t-1})}$ and the following inequality
    \begin{align}
        &\iint(p_{t-1}-p_{t-2})(x)f(x,y)(q_{t-1}-q_{t})(y)dxdy\notag
        \\
        \leq&\|p_{t-1}-p_{t-2}\|_{TV}\left\|\int f(\cdot,y)(q_{t-1}-q_{t})(y)dy\right\|_{L^{\infty}}\notag
        \\
        \leq&\|p_{t-1}-p_{t-2}\|_{TV}\|q_{t-1}-q_{t}\|_{L^1}.
    \end{align}
    Combining the above two inequalities in \eqref{main-estimate} and \eqref{part-estimate}, we obtain
    \begin{align}\label{estimation-combination-Q}
        \sum_{t=1}^k\gamma_t Q(w_t,w)\leq&\gamma_1\eta_1 \mathrm{KL}(p\|p_0)-\gamma_k(\eta_k+\lambda_2)\mathrm{KL}(p\|p_k)+\gamma_1\tau_1 \mathrm{KL}(q\|q_0)-\gamma_k(\tau_k+\lambda_2) \mathrm{KL}(q\|q_k)\notag
        \\
        &-\gamma_k\eta_k\mathrm{KL}(p_k\|p_{k-1})-\gamma_k\iint(p_k-p_{k-1})(x)f(x,y)(q_k-q)(y)dxdy+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon\notag
        \\
        &+\sum_{t=1}^k\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]+(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\}.
    \end{align}
    The result in \eqref{out-layer-result1} then follows from the above inequality and the fact that by \eqref{out-layer-4},
    \begin{align}\label{estimation-pfq}
        &-(\tau_k+\lambda_2)\mathrm{KL}(q\|q_k)-\eta_k\mathrm{KL}(p_k\|p_{k-1})-\iint(p_k-p_{k-1})(x)f(x,y)(q_k-q)(y)dxdy\notag
        \\
        \leq&-(\tau_k+\lambda_2)\mathrm{KL}(q\|q_k)-\eta_k\mathrm{KL}(p_k\|p_{k-1})+\sqrt{\mathrm{KL}(p_k\|p_{k-1})}\sqrt{\mathrm{KL}(q\|q_k)}\notag
        \\
        \leq&-\left(\tau_k+\lambda_2-\frac{1}{4\eta_k}\right)\mathrm{KL}(q\|q_k)
    \end{align}
    Fixing $w=w^*$ in the above inequality \eqref{estimation-combination-Q} when combining \eqref{estimation-pfq} and using the fact that $Q(w_t,w^*)\geq 0$, we obtain \eqref{out-layer-result2}. Finally, \eqref{out-layer-result3} is concluded from similar ideas and a different bound
    \begin{align}
        &-(\tau_k+\lambda_2)\mathrm{KL}(q\|q_k)-\eta_k\mathrm{KL}(p_k\|p_{k-1})-\iint(p_k-p_{k-1})(x)f(x,y)(q_k-q)(y)dxdy\notag
        \\
        \leq&-(\tau_k+\lambda_2)\mathrm{KL}(q\|q_k)-\eta_k\mathrm{KL}(p_k\|p_{k-1})+\sqrt{\mathrm{KL}(p_k\|p_{k-1})}\sqrt{\mathrm{KL}(q\|q_k)}\notag
        \\
        \leq&-\left(\eta_k-\frac{1}{4(\tau_k+\lambda_2)}\right)\mathrm{KL}(p_k\|p_{k-1}).
    \end{align}
\end{proof}



In order to guarantee the convergence of density ratio (Appendix \ref{Langevin-error}), we introduce the super log-Sobolev inequality. \congfang{???}
\begin{definition}
    We say that density $p$ satisfies super log-Sobolev inequality if there exists a monotonically non-increasing function $\beta:(0,\infty)\rightarrow\mathbb{R}$ such that
    \begin{align}
        \mathbb{E}_p[g^2\log(g^2)]\leq r\mathbb{E}_p[\|\nabla g\|^2]+\mathbb{E}_p[g^2]\log(\mathbb{E}_p[g^2])+\beta(r),
    \end{align}
    for all $r>0, g\in\mathcal{D}(\Gamma)$ where $\Gamma$ is a bilinear map\, (there is a brief introduction in Appendix \ref{Langevin-error}).
\end{definition}

%The super log-Sobolev inequality indicates the convergence of density ratio .
 In this paper, the target densities in each mirror (proximal) step to be sampled satisfy the super log-Sobolev inequality with $\beta(r)=C'-c'\log(r/2)$ which implies that $p$ satisfies LSI \eqref{LSI} with constant $\alpha=2e^{-\frac{C'}{c'}}$ as well.


==> parts/method.tex <==

\section{Preliminary}\label{sec:preli}

\paragraph{Notation.} We use lower-case letters $x, y$ to denote
vectors. For function $f:\RR^d\rightarrow\RR$, 
$\nabla f(\cdot)$ and $\nabla^2 f(\cdot)$ denote its gradient and  Hessian matrix, respectively. 
For function $f:\RR^d\rightarrow\RR^d$, $\nabla f(\cdot)$ denotes the
Jacobian matrix.
For multivariate function $f(x,y)$, $\nabla_x$, $\nabla_y$ denote the gradient over $x$, $y$.
Notation $\Vert\cdot\Vert$ denotes 2-norm for both vector and matrix. 
The continuous probability measures in this paper are considered to be absolutely continuous by default with respect to the Lebesgue measure, which induces density function $p$ and $q$. The smoothness is guaranteed by Gaussian initialization and Gaussian smoothing during the updates.
For twice differentiable function $f:\RR^d\rightarrow\RR$, we say that $f$ is $L_0$-Lipschitz if  $|f(x)-f(y)|\leq L_0 \Vert x-y\Vert$ for any $x,y\in\RR^d$; we say that $f$ has $L_1$-Lipschitz gradient if $\|\nabla f(x)-\nabla f(y)\|\leq L_1 \Vert x-y\Vert$ for any $x,y\in\RR^d$. For any a topological space  %we say that $f$ has $L_2$-Lipschitz Hessian if $\|\nabla^2 f(x)-\nabla^2 f(y)\|\leq L_2 \Vert x-y\Vert$ for any $x,y\in\RR^d$
$\mathcal{X}$, $\mathcal{P}(\mathcal{X})$ denotes set of probability measures on $\cX$ and 
$\mathcal{P}_2(\mathcal{X})$ denotes the set of probability measures with bounded second moments.
For density $p$, we define $\cE(p)=\mathbb{E}_p[\log(p)]$, $\mathrm{KL}(p\|q)=\mathbb{E}_p[\log (p/q)]$. For the generalized density for particles, we use Dirac delta distribution $\dirac_{x}$ to represent the Dirac delta distribution at $x$, $\dirac_{\{x_1,\cdots,x_n\}} = n^{-1}\sum_{i=1}^n\dirac_{x_i}$.



%%where $R(\cdot)$ is a density regularizer.
\paragraph{Problem Setup.}
Assume that the min-max problem is defined on the joint parameter space $\cX \times \cY$ and a payoff function $f: \cX \times \cY\rightarrow \RR$. 
We consider the bounded function case. For simplicity without loss of generality, the
domain $\cX \times \cY$ is the 
Euclidean space $\RR^m\times\RR^n$ and the co-domain of $f$  is a bounded interval $[-1,1]$. 


In our work, we consider the regularized minimax problem defined in Eq.~\eqref{eq:problem_particle}. For the regularization term,  
we set 
\begin{equation}\label{eq:relative_reg}
\cR(p(x))=\EE_{p(x)}\left[\lambda_1\|x\|^{2}+\lambda_2\log(p(x))\right] 
\end{equation}
where $\lambda_1,\lambda_2>0$ are constants to determine the regularization scaling as well as the variance of the prior.
We use $\cL(p,q)$ to denote $\EE_{p(x)} \EE_{q(y)} f(x,y)  + \cR(p) - \cR(q)$.
%Recall that a pure Nash equilibrium denotes a pair of strategies $(x,y)\in \cX \times \cY$ such that for all $(x',y')\in \cX \times \cY$, $f(x,y') \leq f(x,y)\leq f(x',y)$.  Similarly, 
The mixed Nash equilibrium denotes a distribution pair $(p_*,q_*)$ such that for all $(p,q)\in \cP(\cX )\times \cP(\cY)$, $\cL(p_*,q) \leq \cL(p_*,q_*)\leq \cL(p,q_*)$.   \congfang{Note $\lambda_1$ and $\lambda_2$ can be arbitrarily small.
Intuitively, $\lambda_1$ brings quadratic growth for the log-density tail and $\lambda_2$ control the amount of uncertainty.
A degenerate $\lambda_2$ will cause the curse of dimensionality for the running time complexity, which is proved to be unavoidable \citep{daskalakis2009complexity,daskalakis2013complexity}.}

\paragraph{Assumptions.}
\begin{enumerate}[label={\textbf{[A$_\text{\arabic*}$]}}]
    \item There exists $L_0$ such that $f$ is $L_0$-Lipschitz.\label{ass:a1}
    \item $f$ has $L_1$-Lipschitz gradient.\label{ass:a2}
 \item For any $x,y\in \cX\times\cY$, $| f(x,y)|\leq 1$.\label{ass:a4}
\end{enumerate}

We consider the bounded function with growth regularities. The bound of $|f|$ is chosen as 1 for notation simplicity.
Assumption \ref{ass:a1}, \ref{ass:a2} regularize the growth of $f$, $\nabla f$ respectively and the definition of  Lipschitz continuity was introduced in \textbf{Notation} part. It is clear that our assumption is quite weak so  our setting is general.
%$\nabla^2 f$


\paragraph{Primal-Dual Algorithms for Min-Max Optimization.}
Primal-Dual method is a classical approach to solve saddle point problems \citep{nemirovski2004prox,he2017algorithmic,lan2020first,bredies2015preconditioned,luke2018globally}. For example, consider the min-max problem
\begin{align}\label{saddle-point-problem}
    \min_{x\in \cX}\max_{y\in \cY}\left\{f(x)+\langle Ax,y\rangle-g(y)\right\},
\end{align}
where $A\in\mathbb{R}^{m\times n}$ denotes a linear mapping, and $f:\cX\rightarrow \mathbb{R}$ and $g:\cY\rightarrow \mathbb{R}$ are two convex functions. General optimization problems with linear constraints: $\min\limits_{x\in\cX}\{f(x):Ax=b \}$ \congfang{can be transformed to}
%is a special case covered by
Eq.~\eqref{saddle-point-problem}. The proximal primal-dual algorithm updates $x_t$ and $y_t$ according to
\begin{align}
    \Tilde{x}_t=&x_{t-1}+\mu_t(x_{t-1}-x_{t-2}),
    \\
    y_t=&\arg\min\limits_{y\in\cY}\langle-A\Tilde{x}_t,y\rangle+g(y)+\tau_t W(y_{t-1},y),
    \\
    x_t=&\arg\min\limits_{x\in\cX}\langle y_t,Ax\rangle+f(x)+\eta_t V(x_{t-1}, x),
\end{align}
under a finite dimension condition with $W$ and $V$ representing Bregman's distances on $\cY$ and $\cX$, respectively. Moreover, $\{\tau_t\}, \{\eta_t\}, \{\gamma_t\}$ are algorithmic parameters to be specified.  The
Bregman divergence is particularly important for other Riemannian structures.
In probability space, the Bregman divergence is usually chosen as KL divergence or Wasserstein distance.

%Specially, the accelerated gradient descent method in can be viewed asa special case of the above primal-dual method \cite{lan2020first}.
 



\paragraph{Unadjusted Langevin Algorithm.} We introduce the 
\emph{Unadjusted Langevin Algorithm (ULA)}
to solve the mirror steps in our setting. In particular, some isoperimetry inequalities shall be introduced to make each step well-posed.


\begin{definition} \citep{gross1975logarithmic}
We say that density $p$ satisfies log-Sobolev inequality (LSI) with a constant $\alpha>0$, if
\begin{align}\label{LSI}
    \mathbb{E}_{p}[g^2\log(g^2)]-\mathbb{E}_{p}[g^2]\log\mathbb{E}_{p}[g^2]\leq\frac{2}{\alpha}\mathbb{E}_{p}[\|\nabla g\|^2]
\end{align}
for all differentiable function $g$ with 
 $\mathbb{E}_{p}[g^2]<\infty$. When $g = \sqrt{p/q}$, we have 
$
\mathrm{KL}(p\Vert q) \leq \frac{1}{2\alpha} \EE_p \left\Vert \nabla \log \frac{p}{q}\right\Vert^2.
$
\end{definition}

Assume we aim to sample from a smooth target probability density $p\propto e^{-f(x)}$ where $f(x)$ has $L_1$-Lipschitz gradient and satisfies a smoothness condition. The ULA with step size $\epsilon>0$ is the discrete-time algorithm
\begin{align}
    x_{s+1}=x_s-\epsilon\nabla f(x_s)+\sqrt{2\epsilon}\zeta_s,
\end{align}
where $s=0,\cdots,T$ for some positive integer $T$; $x_0$ is given as an initialization;  
$\zeta_s\sim\mathcal{N}(0,I)$ is an isotropic Gaussian noise. Moreover, if $p$ satisfies LSI, we can guarantee that $\rho_s$ converge to 
$p_\epsilon$ with a linear convergence rate in KL divergence under fixed step size, where
$\rho_s$ is the density of  $x_s$ along ULA at step-$s$, and $p_\epsilon$ is a biased stationary distribution.
The $\text{KL}(\rho_s\|p)$ along ULA would also converge to $\cO(\epsilon)$. 
Since it is equivalent with gradient descent with additional Gaussian noise, it is easy to implement in practice. 
Moreover, 
the asymptotic bias along ULA in KL divergence $\text{KL}(p_\epsilon\|p)$  can be reduced with a sufficiently small step size.
The  easy-to-implement property and the arbitrarily small bias make it a popular in sampling literature. Thus, we choose it to solve our sub-problems.

%As $\epsilon\rightarrow 0$, ULA recovers the Langevin dynamics in continuous-time. 
%to 
%with linear rate
%with the following error bound \citep{vempala2019rapid}\begin{align}    \text{KL}(\rho_s\|p)\leq e^{-\alpha\epsilon s}\text{KL}(\rho_0\|p)+\frac{8\epsilon mL_1^2}{\alpha},\end{align}

%where $\rho_s$ is the probability density of random variable $x_s$ that evolves ULA at step-$s$; $m$ is the dimension; $\epsilon$ denotes the step size.

\iffalse
The ULA with step size $\epsilon>0$ is the discrete-time algorithm
\begin{align}
    x_{s+1}=x_s-\epsilon\nabla f(x_s)+\sqrt{2\epsilon}\zeta_s,
\end{align}
where $s=0,\cdots,T$ for some positive integer $T$; $x_0$ is given as initialization;  
$\zeta_s\sim\mathcal{N}(0,I_m)$ is an isotropic Gaussian noise drawn in $\mathbb{R}^m$. Specifically, we can write $s$-th step of ULA \eqref{Langevin-dynamic-main-text} as the output at time $\epsilon$ of the stochastic differential equation
\begin{align}\label{eq:disc}
    dx_{s+t}=- \epsilon\nabla f(x_{s})dt+\sqrt{2\epsilon}dW_t^m,\quad t\in[0,1]
\end{align}
where  $\epsilon$ is the step size and $W_t^m$ is the standard Brownian motion in $\mathbb{R}^m$ starting at $W_0^m=0$. 
Eq.~\eqref{eq:disc} represents the discretized Langevin dynamics.


The continuous version evolves  as following
\begin{align}\label{Langevin-dynamic-main-text}
    dx_{s+t}=-\epsilon\nabla f(x_{s+t})dt+\sqrt{2\epsilon}dW_t^m, \quad t\in[0,1]
\end{align}
where $\epsilon$ is the step size and $W_t^m$ is the standard Brownian motion in $\mathbb{R}^m$ starting at $W_0^m=0$. 
\fi
%$\nabla f(x_{s+t})$ is a time-dependent drift force in each interval. 






\begin{algorithm*}[t]
\caption{Particle-based Primal-Dual Algorithm for Mixed Nash Equilibrium} \label{alg:algorithm}
\hspace*{0.02in} {\bf Input:} 
 number of outer iterations $T$, outer-loop learning rates $\{\eta_t\}_{t=1}^T$ and $\{\tau_t\}_{t=1}^T$,  outer-loop hyper-parameters $\{\mu_t\}_{t=1}^T$; number of inner iterations $\{T_t\}_{t=1}^T$, inner-loop learning rates $\{\iota_t\}_{t=1}^T$, 
 number of particles $M$
 \\
\hspace*{0.02in} {\bf Output:} estimated equilibrium   
$(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}})$

\begin{algorithmic} 
\STATE Initialize parameters $\{\Tilde{x}_r^{(0)}\}_{r=0}^M\sim p_0(x)\propto\exp\left\{-\frac{\lambda_1}{\lambda_2}\|x\|^2\right\},\ \{\Tilde{y}_r^{(0)}\}_{r=0}^M\sim q_0(y)\propto\exp\left\{-\frac{\lambda_1}{\lambda_2}\|y\|^2\right\}.$ 

Assign $(\tilde{X}^{(-1)},\tilde{Y}^{(-1)})=(\tilde{X}^{(0)},\tilde{Y}^{(0)})\leftarrow\left(\{\Tilde{x}_r^{(0)}\}_{r=1}^M, \{\Tilde{y}_r^{(0)}\}_{r=1}^M\right)$.

Assign $h^{(0)}(y) = \frac{\lambda_1}{\lambda_2}\|y\|^2 $, $g^{(0)}(x) = \frac{\lambda_1}{\lambda_2}\|x\|^2 $.
\FOR{$t=0$ to $T-1$}
    \STATE Initialize $(X^{(0)},Y^{(0)})\sim p_0(x)\times q_0(y)$.
    \STATE Update $
    h^{(t+1)}(y) 
    =\frac{1} {\lambda_2+\tau_{t+1}}\left\{\hat{\phi}_{t+1}(y)
+\lambda_1\|y\|^{2}+\tau_{t+1}h^{(t)}(y)\right\}.
    $
    \FOR{$k=0$ to $T_t$, $r=0$ to $M$}
        %\STATE for $r\in\{1,2,\cdots,M\}$
        %\STATE $\nabla_y h^{(t+1)}(y)=\frac{1} {\lambda_2+\tau_{t+1}}\left\{\int \nabla_y f(x, y)[\mu_{t+1}p_{t-1}-(1+\mu_{t+1})p_{t}](x)dx+(2)\lambda_1\|y\|^{\delta}y\right\}+\frac{\tau_{t+1}}{\lambda_2+\tau_{t+1}}\nabla_y h^{(t)}(y)$
        \STATE Run noisy gradient descent 
        $y_r^{(k+1)}\leftarrow y_r^{(k)}-\iota_t\nabla_y h^{(t+1)}(y_r^{(k)})+\sqrt{2\iota_t}\xi_r^{(k)}$, where $\xi_r^{(k)}\sim\mathcal{N}(0, I_{n})$.
    \ENDFOR
    \STATE Assign $\Tilde{Y}^{(t+1)}\leftarrow Y^{(T_t+1)}$.
    \STATE Update $
    g^{(t+1)}(x)
    =\frac{1} {\lambda_2+\eta_{t+1}}\left\{\hat{\psi}_{t+1}(x)+\lambda_1\|x\|^{2}+\eta_{t+1} g^{(t)}(x)\right\}.
    $
    
    \FOR{$k=0$ to $T_t$, $r=0$ to $M$}
        %\STATE  for $r\in\{1,2,\cdots,M\}$
        %\STATE $\nabla_x g^{(t+1)}(x)=\frac{1} {\lambda_2+\eta_t}\left\{\int\nabla_x f(x,y)q_{t+1}(y)dy+(2)\lambda_1\|x\|^{\delta}x\right\}+\frac{\eta_t}{\lambda_2+\eta_t}\nabla_x g^{(t)}(x).$
        \STATE Run noisy gradient descent $x_r^{(k+1)}\leftarrow x_r^{(k)}-\iota_t\nabla_x g^{(t+1)}(x_r^{(k)})+\sqrt{2\iota_t}\zeta_r^{(k)}$, where $\zeta_r^{(k)}\sim\mathcal{N}(0, I_{m})$.
    \ENDFOR
    \STATE Assign $\Tilde{X}^{(t+1)}\leftarrow X^{(T_t+1)}$.
    
\ENDFOR 

\textbf{Option I:} $
(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}}) \leftarrow 
(\frac{1}{M}\dirac_{\Tilde{X}^{(T)}},\frac{1}{M}\dirac_{\Tilde{Y}^{(T)}})$.

\textbf{Option II:} Randomly pick up $t\in\{1,\cdots,T\}$ following the probability $\mathbb{P}[t]=\frac{\mu_t}{\sum_{t=1}^T\mu_t}$ as $(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}})$.
\end{algorithmic}
\end{algorithm*}



\section{Particle-based Primal-Dual Algorithm}
We propose Particle-based Primal-Dual Algorithm (PAPAL) to solve the regularized minimax problem Eq.~\eqref{eq:problem_particle} by applying Unadjusted Langevin Algorithm (ULA) to Mirror-Prox Primal-Dual method.
%\congfang{???} In particular, we introduce the Langevin dynamics convergence of our method to illustrate the algorithmic intuition and develop the convergence analysis for infinite-dimension mirror-prox on probability measures using the bound on density ratio in sub-problem.\congfang{???}

As an optimization algorithm on the space of  continuous probability measures, our proposed PAPAL (Algorithm \ref{alg:algorithm}) consists of two components: inner loop and outer loop. Specifically,
our outer loop extends the classical primal-dual scheme (Sec. \ref{sec:preli}) to infinite dimensional optimization problems (Sec. \ref{sec:pd}). Each outer step can be rewriten as a sampling task for Gibbs distribution (Sec. \ref{sec:energy}). We perform ULA as the inner loop to approximate a proximal Gibbs distribution, which is applied to the outer loop optimization to converge to the Mixed Nash Equilibrium distributions $p^*$ and $q^*$ (Sec. \ref{sec:solver}). We will provide the motivation of our algorithm from an optimization view (Sec. \ref{sec:opt_view}).

% In the following parts, we will provide the interpretation and motivation of our algorithm thoroughly.

\subsection{Exact Primal-Dual Method}\label{sec:pd}


%and approximate them by some inner loops
We construct the target density of $p^*_t$ and $q^*_t$ for each iteration. Particularly, given $\hat{p}_{-1}$, $\hat{p}_0$, and $\hat{q}_0$,
$q_t^*(y)$ and $p_t^*(x)$ satisfy the following recursive condition,
    \begin{align}              
q_t^*:=&\argmin_{q\in\cP_2(\cY)}\mathbb{E}_q[\hat{\phi}_t(y)]+\cR(q) +
        \tau_t \mathrm{KL}(q\|q_{t-1}^*), \label{minimizer-q}
        \\ p_t^*:=&\argmin_{p\in\cP_2(\cX)}\mathbb{E}_p[\hat{\psi}_t(x)]+\cR(p)
        +\eta_t \mathrm{KL}(p\|p_{t-1}^*), \label{minimizer-p}
    \end{align}
    where $\hat{\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{\hat{p}_{t-1}}[f(\cdot,y)]+\mu_t\mathbb{E}_{\hat{p}_{t-2}}[f(\cdot,y)]$, and $\hat{\psi}_t(x)=\mathbb{E}_{\hat{q}_t}[f(x,\cdot)]$. 

    If $\hat{q}_t = q_t^*$, $\hat{p}_t = p_t^*$, Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} perform exact primal-dual method in continuous probability space, with KL divergence as the Bregman divergence. However,
    there two gaps for the aforementioned updates: 
    (1) the forms of $q_{t-1}^*$ and $p_{t-1}^*$ are not explicit in Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p};
    (2) the exact solutions for $\hat{q}_t$ and $\hat{p}_t$ are not tractable.
    Thus, it is necessary to derive to feasible form of $(q_{t-1}^*,p_{t-1}^*)$ and approximate the optimal $(q_t^*,p_t^*)$.

    
    %\paragraph{Remark.} We would like to distinguish 
    %\hanze{\\TBA \\ more clear clarification about $p^*_t$, $p_t$, and $\hat{p}_t$\\(Monte Carlo)}

    %the computation and update on particles should still be adapted. 

\subsection{Recursive Energy Function}\label{sec:energy}

Section \ref{sec:pd} provides us an algorithm to find mixed Nash equilibrium in the probability space.
In this part, we would discuss the feasibility of the proposed updates.

%Importantly, the loss function Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} include $q_*^{t-1}$ and $p_*^{t-1}$ term, which are not explicit in an algorithm.
The following Lemma provides us insight to obtain the explicit form of $q_*^{t-1}$ and $p_*^{t-1}$ in  Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} recursively, which can be implemented in an algorithm.


\begin{lemma}\label{lemma:optimal-KL-prox}
    Let $\lambda>0$ be a positive real number and $\tilde{l}(\theta), l(\theta)$ be bounded continuous functions. Consider a probability density $\Bar{p}(\theta)\propto\exp\left(-\tilde{l}(\theta)\right)$, then $p(\theta)\propto\exp\left(-\frac{1}{\lambda+\tau}l(\theta)-\frac{\tau}{\lambda+\tau}\tilde{l}(\theta)\right)$ is an optimal solution to the following problem  
    \begin{align}
        \min\limits_{p\in\mathcal{P}_2}\{\mathbb{E}_{p}[l(\theta)]+\lambda \cE(p)+\tau \mathrm{KL}(p\|\Bar{p})\}.
    \end{align}
\end{lemma}

Once we obtained two approximate distributions
$\hat{p}_i(y)$ and $\hat{p}_i(x)$, Lemma \ref{lemma:optimal-KL-prox} indicates that if $p_{t-1}^*$ and $q_{t-1}^*$ are proximal Gibbs distribution
with explicit form. 
Then, $p_t^*$ and $q_t^*$ have the similar expression as well. Therefore, we denote 
    \begin{align*}
    h^{(t)}(y) 
    =\frac{1} {\lambda_2+\tau_t}\left\{\hat{\phi}_t(y)
+\lambda_1\|y\|^{2}+\tau_th^{(t-1)}(y)\right\},
    \\
    g^{(t)}(x)
    =\frac{1} {\lambda_2+\eta_t}\left\{\hat{\psi}_t(x)+\lambda_1\|x\|^{2}+\eta_t g^{(t-1)}(x)\right\}.
    \end{align*}

    % $h^{(t)}(y):=\sum_{i=1}^t a_{i}^t\left\{\mu_{i}\mathbb{E}_{p_{i-2}}[f(\cdot,y)]-\right.\\
    % \left.(1+\mu_i)\mathbb{E}_{p_{i-1}}[f(\cdot, y)]\right\}+\sum_{i=1}^t
    % a_{i}^t\|y\|^{2}+\frac{a_{1}^t\tau_1}{\lambda_2}\|y\|^2$ and $a_{i}^t=\frac{\lambda_1}{\lambda_2+\tau_i}\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}$
    
    % $g^{(t)}(x):=\sum_{i=1}^t b_{i}^t\mathbb{E}_{q_i}[f(x,\cdot)]+\sum_{i=1}^t b_{i}^t\|x\|^{2}+\frac{b_{1}^t \eta_1 }{\lambda_2}
    % \|x\|^2$ and $b_{i}^t=\frac{\lambda_1}{\lambda_2+\eta_i}\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}$
    
    which consist of the Gibbs potential on $\mathcal{P}_2(\mathcal{Y})$ and $\mathcal{P}_2(\mathcal{X})$ after $t-1$ iterations. Thus, at each step-$t$, our objective probability densities can be written as 
    \begin{align}
        q_t^*(y)=\frac{\exp\left(-h^{(t)}(y)\right)}{Z_{t,1}},\, \, \, \, p_t^*(x)=\frac{\exp\left(-g^{(t)}(x)\right)}{Z_{t,2}},\notag
    \end{align}
    where $Z_{t,1}$ and $Z_{t,2}$ are normalizing constants. 
%(the approximate probability densities we obtain are $q_t(y)$ and $p_t(x)$)
%\subsection{Particle Approximation}

\subsection{Inexact Solver and Particle Approximation}\label{sec:solver}

For each step-$t$, the ideal case ($\hat{q}_t = q_t^*$, $\hat{p}_t = p_t^*$) is not tractable in the algorithm. Since there is not closed form to compute Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}.
Fortunately, the optimization of random variables can be approximately done given the log density. ULA is a widely algorithm to approximate the target distribution. After several steps, 
$(q_t,p_t)$ can be obtained to approximate $(q^*_t,p^*_t)$. Thus, $\hat{q}_t = q_t$ and $\hat{p}_t = p_t$ lead to an approximated algorithm given Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}. Nonetheless, the realization of $(q_t,p_t)$ pair can only be executed a finite number of times. Thus, the $(q_t,p_t)$ pair in an algorithm should be a pair of particle sample sets, which is denoted as $(\hat{q}_t,\hat{p}_t)$.
Specifically, the full procedure can be done as follows.

We first initialize a set of particles and duplicate it  $\{x_r^{(-1)},y_r^{(-1)}\}_{r=1}^M =\{x_r^{(0)},y_r^{(0)}\}_{r=1}^M
$. 
For each step, we run ULA to optimize the particles in $\cY$,  where the gradient at the $k$-th inner step is given by $\nabla_y h^{(t)}(y_r^{(k)})$ estimated by $x_r^{(k-1)}$ and $x_r^{(k-2)}$. Then, we execute the same process as above starting from the prior where the gradient at the $k$-th inner step is given by $\nabla_y g^{(t)}(x_r^{(k)})$ estimated by $y_r^{(k-1)}$. The reason why we run the Langevin algorithm on $\mathcal{P}_2(\mathcal{Y})$ firstly is that the approximate probability density $q_t(y)$ (or $\hat{q}_t(y)$) is necessary for the $t$-th optimization step on $\mathcal{P}_2(\mathcal{X})$.

Thus, we obtain the full procedure of PAPAL in Algorithm \ref{alg:algorithm}. We also provide empirical results in Appendix \ref{sec:empi}.



%Another intractable term in the algorithm is the gap

\paragraph{Remark 1.} In the following parts, to make a clear
distinction between  $(\hat{q}_t,\hat{p}_t)$, $(q_t,p_t)$, and $(q^*_t,p^*_t)$, we reiterate the definition here: we initialize $(\hat{q}_{-1},\hat{p}_{-1})=(\hat{q}_0,\hat{p}_0)$ from the prior distribution. From $t=1$ to $t=T$, $(q^*_t,p^*_t)$ is the exact solution from Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}; $(q_t,p_t)$ is the ULA approximation of $(q^*_t,p^*_t)$;  $(\hat{q}_t,\hat{p}_t)$ is the realization of $(q_t,p_t)$ with $M$ samples (mixture of dirac delta distributions). All the densities above can be defined by recursion.


\paragraph{Remark 2.} There are other sampling algorithms can be implemented here as the inexact solver, such as Hamiltonian Monte Carlo \citep{duane1987hybrid,neal2011mcmc}, Metropolis-adjusted Langevin algorithm  \citep{rossky1978brownian,grenander1994representations}.
We use ULA here for demonstration and simplicity. More sophisticated solvers can usually improve the convergence speed.




\subsection{Optimization View of PAPAL}\label{sec:opt_view}

In this subsection we explain the algorithmic intuition behind PAPAL from an optimization perspective. Recall that Algorithm \ref{alg:algorithm} iteratively updates the particles $\hat{q}_t$ and $\hat{p}_t$ which the approximate the minimizers of the linearized potentials Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}. 
Actually, we obtain the classical Primal-Dual algorithm  \citep{nemirovski2004prox} if Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} degenerate to finite dimension. It is obvious that we can find $q_t^*$ and $p_t^*$ with negligible error under finite dimension condition which implies the total complexity would be derived easily. 
However, there are three problems if we rely on Langevin algorithm when solving the sub-problem for infinite dimension: 

(1)  Express the objective densities of the sub-problem as the form of $e^{-h^{(t)}(y)}/Z_{t,1}$ and $e^{-g^{(t)}(x)}/Z_{t,2}$, which can be explicitly obtained in an algorithm;

(2) Analysis the outer loop
    with the bounded KL error induced by ULA at each step-$t$, which converges linearly with fixed step size under LSI;
    
(3) Control the error induced by finite particles at each step-$t$, which should be done by concentration;



The first problem can be solved by forward recursion of $(q_{t-1}^*,p_{t-1}^*)$ and Lemma \ref{lemma:optimal-KL-prox} combining the approximated solutions $\left\{(\hat{q}_k, \hat{p}_k)\right\}_{k=-1}^{t-1}$ we have known.
Next, in order to bound the error between approximate densities and precise densities in each iteration of Primal-Dual method, we introduce the LSI condition \citep{gross1975logarithmic}, which can guarantee the fast convergence of sampling algorithms, such as ULA.
Therefore, we add $\|\cdot\|^{2}$ term with coefficient $\lambda_1$, ($\lambda_1$ can be an arbitrary positive number) to the regularizer which guarantee that $q_t^*$ and $p_t^*$ satisfy the LSI condition. 
Finally, the finite particle $\hat{\phi}_t$ and $\hat{\psi}_t$ approximate the true expectation 
${\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{{p}_{t-1}}[f(\cdot,y)]+\mu_t\mathbb{E}_{{p}_{t-2}}[f(\cdot,y)]$, and
$ {\psi}_t(x)=\mathbb{E}_{{q}_t}[f(x,\cdot)]$. The gap between $(\hat{\phi}_t,\hat{\psi}_t)$ and $({\phi}_t,{\psi}_t)$ shall be controlled by concentration techniques.



To sum up, we connect bilinear forms $\langle Ax,y\rangle$ under finite dimension and $\EE_{p(x)}\EE_{q(y)}f(x,y)$ under infinite dimension with proximal Gibbs distribution. In addition, we apply the estimation of sub-problem error and finite sample error 
to global convergence analysis for our particle-based algorithm. Therefore, we may interpret the PAPAL as a finite-particle approximation of a primal-dual method. PAPAL combines the efficient convergence of Primal-Dual method in outer loop and the KL error bound of ULA under LSI condition in inner loop. More importantly, the loss functional can be estimated with polynomial finite particles, which makes our algorithm implementable.

%\congfang{moderate number of particles???}


\section{Convergence Analysis}
In this section,  we provide quantitative global convergence for PAPAL. %in discrete time.
We first provide the finite sample error bound in Sec.~\ref{sec:finite}.
Then, we
introduce the outer loop settings in Sec.~\ref{subsection-5.1} and conclude the properties of the updates. By assuming the approximate optimality of the inner loop iterations, the error bound of the outer loop can be obtained.
In Sec.~\ref{subsection-5.2}, we 
discuss the convergence rate for the inner loop iterations, which is the KL convergence of ULA algorithm.
 Finally, in Sec.~\ref{subsection-5.3}, we combine the outer loop and the inner loop to discuss the total complexity of PAPAL and provide the 
 global convergence results of our main theorem.

\subsection{Finite Sample Error}\label{sec:finite}
 We concentrate on probability sets $\cQ_{\cX}$ and $\cQ_{\cY}$ as follows
 \begin{align*}
     &\cQ_{\cX}:=\left\{p(x)\propto e^{-l_1(x)-\frac{\lambda_1}{\lambda_2}\|x\|^2}; \|l_1\|_\infty\leq \frac{C}{\lambda_2}\right\},\\
     &\cQ_{\cY}:=\left\{q(y)\propto e^{-l_2(y)-\frac{\lambda_1}{\lambda_2}\|y\|^2};\|l_2\|_\infty\leq \frac{C}{\lambda_2}\right\},
 \end{align*}
 for a fixed positive constant $C$. According to the form of objective function in Eq.~\eqref{eq:problem_particle}, we just need to bound the discretization error on linear term. Therefore, we use the following lemma to bound the discretization error between $\hat{p}_t$ and $p_t$ ($\hat{q}_t$ and $q_t$) at each step-$t$ (Appendix \ref{discre}).
 \begin{lemma}
     The errors of finite particles satisfy
     \begin{align}
         &\mathbb{P}\left[\left|(\hat{p}_t-p_t)(x)f(x,y)q(y)dydx\right|\geq\epsilon\right]\leq\delta,
         \\
         &\mathbb{P}\left[\left|(\hat{q}_t-q_t)(y)f(x,y)p(x)dxdy\right|\geq\epsilon\right]\leq\delta,
     \end{align}
     with the required numbers of particle $M:=\mathcal{O}\left(\epsilon^{-2}\left[-\log(\delta)+d\log(1+\sqrt{\lambda_2/\lambda_1}\epsilon^{-1})\right]\right)$ 
     on $\hat{p}_t(x)$ and $\hat{q}_t(y)$ for all $p(x)\in\cQ_{\cX},\, q(y)\in\cQ_{\cY}$ where $d=\max\{m,n\}$ is the dimension.
 \end{lemma}

\subsection{Outer Loop Error Bound}\label{subsection-5.1}
We introduce the Max-Min gap function 
\begin{align}
    Q(\Bar{w},w):=\mathcal{L}(\Bar{p},q)-\mathcal{L}(p,\Bar{q}),
\end{align}
where $\Bar{w}:=(\Bar{p},\Bar{q})$ and $w:=(p,q)$. It is notable that $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\geq0$ uniformly over $\Bar{w}\in\cP_2(\cX)\times\cP_2(\cY)$ and equality only holds when $\Bar{w}$ arrives at the mixed Nash equilibrium $w_*=(p_*,q_*)$. 

Specially, under the expression of objective function in Eq.~\eqref{eq:problem_particle} and \eqref{eq:relative_reg}, we have
\begin{equation}\label{Max-Min-gap-control-entropy}
\begin{split}
&\max_{w}Q(\Bar{w},w)\geq\lambda_2(\mathrm{KL}(\Bar{p}\|\Bar{p}^*)+\mathrm{KL}(\Bar{q}\|\Bar{q}^*)),\\
&\text{s.t.} \quad\Bar{w}^*=(\Bar{p}^*,\Bar{q}^*)=\argmax_{w'}Q(\Bar{w},w')
\end{split}
\end{equation}
where the domain of $w,w'$ is $\cP_2(\cX)\times\cP_2(\cY)$.
Thus, the Max-Min gap function $Q(\Bar{w},w)$ can control the upper bound of the KL divergence.

To capture the error of our algorithm, we assume that the KL divergence between $(q_t,p_t)$ and $(q^*_t,p^*_t)$ can be bounded by a small error, i.e.,
$$\mathrm{KL}(p_t\|p_t^*)\leq\delta_{t,1},\quad\mathrm{KL}(q_t\|q_t^*)\leq\delta_{t,2},$$
which is guaranteed by ULA algorithm with small step sizes. We use the 
error bound quantities $\delta_{t,1}$
and $\delta_{t,2}$ to analyze the outer loop properties. The following theorem proves the general convergence properties of mirror-prox primal-dual method with an inexact solver.
 %Next, we need to control a set of quantities of error bound for $p_t$ and $q_t$ in the inner loop, 
% \begin{theorem}\label{main-text-outer-loop-thm}
% After $T$ iterations of Primal-Dual method 
% with setting $\gamma_t\mu_t=\gamma_{t-1}$,\,  $\gamma_t\tau_t\leq\gamma_{t-1}(\tau_{t-1}+\lambda_2)$,\, $\gamma_t\eta_t\leq\gamma_{t-1}(\eta_{t-1}+\lambda_2)$,\, $\tau_t\eta_{t-1}\geq\mu_t$ for any $t\geq1$ and the sub-problem errors have been bounded by $\delta_{t,1}(p),\delta_{t,1}(q);\delta_{t,2}(p),\delta_{t,2}(q)$ mentioned above, the estimation of Max-Min gap satisfies
% \begin{align}
%     &\sum_{t=1}^T\gamma_t Q(w_t,w)\notag
%     \\
%     \leq&\gamma_1\eta_1\mathrm{KL}(p\|p_0)-\gamma_T(\eta_T+\lambda_2)\mathrm{KL}(p\|p_T)\notag
%     \\
%     &+\gamma_1\tau_1\mathrm{KL}(q\|q_0)-\gamma_T\left(\tau_T+\lambda_2-\frac{1}{4\eta_T}\right)\mathrm{KL}(q\|q_T)\notag
%         \\
%         &+\sum_{t=1}^T\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]\notag
%         \\
%         &\, \, \, \, \, \, \, \,  +(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\}.
% \end{align}
% \end{theorem}
\begin{theorem}\label{main-text-outer-loop-thm}
By setting parameters $\gamma_t\mu_t=\gamma_{t-1}$,\,  $\gamma_t\tau_t\leq\gamma_{t-1}(\tau_{t-1}+\lambda_2)$,\, $\gamma_t\eta_t\leq\gamma_{t-1}(\eta_{t-1}+\lambda_2)$,\, $\tau_t\eta_{t-1}\geq\mu_t,\, \mu_t\leq 1$ for any $t\geq1$ and optimizing the sub-problem with errors bounded by $\delta_{t,1}, \delta_{t,2}$ mentioned above, iterates of our method satisfies
\begin{align*}
    &\sum_{t=1}^T\gamma_t Q(w_t,w)\notag
    \\
    \leq&\ \ \ \ \ \gamma_1\eta_1\mathrm{KL}(p\|p_0^*)-\gamma_T(\eta_T+\lambda_2)\mathrm{KL}(p\|p_T^*)
    \\
    &+\gamma_1\tau_1\mathrm{KL}(q\|q_0^*)-\gamma_T\left(\tau_T+\lambda_2-\frac{1}{4\eta_T}\right)\mathrm{KL}(q\|q_T^*)
        \\
        &+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon
        \\
        &+\sum_{t=1}^k\gamma_t\left[\left(\lambda_2+\frac{2\lambda_1}{\alpha_{p_t^*}}\right)\delta_{t,1}+\left(30+\frac{8\lambda_1\sigma(p_t^*)}{\sqrt{\alpha_{p_t^*}}}\right)\sqrt{\delta_{t,1}}\right]\notag
        \\
        &+\sum_{t=1}^k\gamma_t\left[\left(\lambda_2+\frac{2\lambda_1}{\alpha_{q_t^*}}\right)\delta_{t,2}+\left(34+\frac{8\lambda_1\sigma(q_t^*)}{\sqrt{\alpha_{q_t^*}}}\right)\sqrt{\delta_{t,2}}\right],
\end{align*}
for any $p\in\cQ_{\cX}, q\in\cQ_{\cY}$ with probability at least $1-{\delta}$ for sample size $M=\Tilde{\Theta}(\epsilon^{-2}[\log(T/\delta)+d\log(\epsilon^{-1})])$ in each iteration where $d=\max\{m,n\}$ is the dimension, $\alpha_p$ is the log-Sobolev coefficient of density $p$ and $\sigma(p)$ denotes $(\mathbb{E}_p[\|\theta\|^2])^{1/2}$.
\end{theorem}

Theorem \ref{main-text-outer-loop-thm} captures the estimation of Max-Min gap. By setting proper $\gamma_t$, the convergence rate of $Q$ can be obtained. We can specify the hyper-parameters $\{\tau_t\},\{\eta_t\},\{\gamma_t\}$ and sub-problem error bound $\delta_{t,1},\delta_{t,2}$ for solving the minimax problem \eqref{eq:problem_particle}. 
% Our goal is to show that the Max-Min gap evaluated at the output solution
% \begin{align}
%     \Bar{w}_T=\frac{\sum_{t=1}^T\gamma_t w_t}{\sum_{t=1}^T\gamma_t},\notag
% \end{align}
% will converge to zero. In addition, we can prove a convergence guarantee about $w_T$ and $w_*$ in KL divergence along [Alogorithm Name]. 
Letting the input parameters be
\begin{equation}\label{parameter-setting}
\begin{split}
    &\mu_t = \mu=\frac{1}{2}\left(2+\lambda_2^2-\lambda_2\sqrt{4+\lambda_2^2}\right),
    \\
    &\eta_t=\tau_t=\frac{\lambda_2\mu}{1-\mu},\quad\gamma_t=\mu^{-t},
    \end{split}
\end{equation}
and defining $c(p)=\min\left\{\frac{1}{2}, \alpha_{p}, \frac{\alpha_{p}}{2(\sigma(p))^2}\right\}$, $c(q)=\min\left\{\frac{1}{2}, \alpha_{q}, \frac{\alpha_{q}}{2(\sigma(q))^2}\right\}$ as the upper bound of the inner loop errors $\delta_{t,1}$, $\delta_{t,2}$, we are ready to provide the following result for outer loop error bound of our algorithm with an inexact solver. Notice that $\mu$ in \eqref{parameter-setting} satisfies $\mu\leq1$ and $\mu^2-(2+\lambda_2^2)\mu+1=0$.
\begin{corollary}\label{main-text-outer-loop-complexity}
    Setting the parameters $\gamma_t,\, \eta_t,\, \tau_t,\, \mu_t$ as in Eq.~\eqref{parameter-setting} and assuming the sub-problem error bounds satisfy $\max\{\delta_{t,1},\delta_{t,2}\}\leq\frac{1}{2}\min\{c(p_t^*), c(q_t^*)\}T^{-2J}$ for any fixed positive integer $J$ and $\epsilon>0$ at each step-$t$, then the Max-Min gap between $\Bar{w}_T:=\frac{\sum_{t=1}^T\gamma_t w_t}{\sum_{t=1}^T\gamma_t}$
    and $\bar{w}_T^*:=\arg\max_{w\in\mathcal{P}_2(\mathcal{X})\times\mathcal{P}_2(\mathcal{Y})}Q(\bar{w}_T,w)$ satisfies
    \begin{align}\label{Max-Min-gap}
        0\leq Q(\Bar{w}_T,\bar{w}_T^*)\leq&\frac{\lambda_2\mu^T}{1-\mu}\left[\mathrm{KL}(\bar{p}_T^*\|p_0)+\mathrm{KL}(\bar{q}_T^*\|q_0)\right]\notag
        \\
        &+8\epsilon+(10\lambda_1+\lambda_2+32)T^{-J}.
    \end{align}
    with probability at least $1-{\delta}$ for sample size $M=\Tilde{\Theta}(\epsilon^{-2}[\log(T/\delta)+d\log(\epsilon^{-1})])$ in each iteration where $d=\max\{m,n\}$ is the dimension, $\Bar{w}_T=\frac{\sum_{t=1}^T\gamma_t w_t}{\sum_{t=1}^T\gamma_t}$. Moreover, we also have the KL-divergence convergence
    \begin{align}\label{KL-divergence-convergence}
        &\mathrm{KL}(p_*||p_T^*)+\frac{1}{2}\mathrm{KL}(q_*||q_T^*)\notag
        \\
        \leq&\mu^T[\mathrm{KL}(q_*||q_0^*)+\mathrm{KL}(p_*||p_0^*)]\notag
        \\
        &+\lambda_2^{-1}\left[8\epsilon+(10\lambda_1+\lambda_2+32)T^{-J}\right],
    \end{align}
    and the convergence in the $W_2$ distance as follows
    \begin{equation*}
    \label{Wassenstain-convergence}
    \begin{split}
        &\frac{1}{2}W_2^2(q_T, q_*)+W_2^2(p_T, p_*)
        \\
        \leq&\frac{4}{\min\{\alpha_{p_T^*}, \alpha_{q_T^*}\}}\left\{\mu^{T}\left[\mathrm{KL}(q_*\|q_0^*)+\mathrm{KL}(p_*\|p_0^*)\right]\right.
        \\
    &+\left.\lambda_2^{-1}\left[8\epsilon+(10\lambda_1+\lambda_2+32)T^{-J}\right]\right\}+3T^{-2J},
    \end{split}
    \end{equation*}
    when the optimal solution $w_*=(p_*,q_*)$ of Eq.~\eqref{eq:problem_particle} exists.
    % \begin{align}\label{KL-divergence}
    %     \frac{1}{2}\mathrm{KL}&(q_*\|q_T^*)+\mathrm{KL}(p_*\|p_T^*)\\
    %     &\leq\mu^{T-1}\left[\mathrm{KL}(q_*\|q_0^*)+\mathrm{KL}(p_*\|p_0^*)\right]+\frac{1}{(1-\mu)}[8\epsilon+(2\lambda_1+\lambda_2+16)T^{-J}]. \notag
    % \end{align}
\end{corollary}

% Corollary \ref{main-text-outer-loop-complexity} demonstrates that PAPAL achieves a pair of $\epsilon$ KL divergence accurate solution of the optimal distribution: $\max\{\text{KL}(q_*\|q), \text{KL}(p_*\|p)\}\leq \epsilon$ or a pair of $\epsilon$ Max-Min gap accurate solution of the optimal distribution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}\{Q(\Bar{w},w)\}\leq\epsilon$ after $\max\left\{\left(\frac{4}{(1-\mu)^2\epsilon}\right)^{1/J}, \frac{\log(4[\text{KL}(q_*\|q_0)+\text{KL}(p_*\|p_0)])-\log((1-\mu)\epsilon)}{\log(\mu^{-1})}\right\}$ iterations.

\subsection{Inner Loop Error Bound}\label{subsection-5.2}
It's necessary to evaluate the iteration complexity of ULA in order to guarantee the global convergence. %In other words, we need to conclude the total complexity by taking both the outer loop and inner loop account.

% \begin{corollary}\label{main-text-cor-langevin-dynamic}
%        There exists a $t_0\in[0,1]$ such that $q_{t}(y)$ and $p_{t}(x)$ which denote the probability densities along Langevin dynamic \eqref{Langevin-dynamic-q} and \eqref{Langevin-dynamic-p} for time $t'$ with $t'-t_0\geq\Tilde{\Theta}(\frac{\log(C_0+1)+1}{\alpha})$ with objective $q_t^*(y)$ and $p_t^*(x)$. 
%        \begin{align}
%            dy_s=&-\nabla_y h^{(t)}(y_s)+dW_s^n,\label{Langevin-dynamic-q}
%            \\
%            dx_s=&-\nabla_x g^{(t)}(x_s)+dW_s^m.\label{Langevin-dynamic-p}
%        \end{align}\congfang{???}
%        The sub-problem error bounds satisfy the following evaluation: $\max\{\delta_{t,1}(p),\delta_{t,2}(p),\delta_{t,1}(q),\delta_{t,2}(q)\}\leq\max\{\mathrm{KL}(p_{t-1}\|p_t^*),\, \mathrm{KL}(q_{t-1}\|q_t^*),\, C_0\}e^{-\alpha(t'-t_0)}$ if Assumption \ref{ass:a1} holds. The constants $C_0, \alpha$ are depend on $\lambda_1, \lambda_2, \delta$\, (see Appendix \ref{Langevin-error} for details).
%         % \begin{align}
%         %     \max\left\{\left\|\frac{dp_{t}}{dp_t^*}-1\right\|_{\infty},\, \,  \left\|\frac{dq_{t}}{dq_t^*}-1\right\|_{\infty}\right\}\leq 
%         %     C_0(\lambda_1,\lambda_2,\delta)&e^{-\alpha(\lambda_1,\lambda_2,\delta)(t'-t_0)},\\
%         %     \max\{\mathrm{KL}(p_{t}\|p_t^*),\, \, \mathrm{KL}(q_{t}\|q_t^*)\}\leq e^{-\alpha(\lambda_1,\lambda_2,\delta)t'}\max\{\mathrm{KL}&(p_{t-1}\|p_t^*),\, \, \mathrm{KL}(q_{t-1}\|q_t^*)\}.
%         % \end{align}
%     \end{corollary}
\begin{theorem}\label{main-text-thm-ULA} \citep{vempala2019rapid}
    Assume that $f(\theta)$ is smooth and has $L_1$-Lipschitz gradient, and consider a probability density $p(\theta)\propto\exp{(-f(\theta))}$ satisfying the log-Sobolev inequality with constant $\alpha$, ULA with step size $0<\iota<\frac{\alpha}{4L_1^2}$ satisfies
    \begin{align}
        \mathrm{KL}(\rho_k||p)\leq e^{-\alpha\iota k}\mathrm{KL}(\rho_0||p)+\frac{8\iota d_\theta L_1^2}{\alpha}
    \end{align}
    where $d_\theta$ is the dimension.
\end{theorem}


\subsection{Global Convergence}\label{subsection-5.3}
We can now conclude the global convergence of PAPAL using Corollary \ref{main-text-outer-loop-complexity} and Theorem \ref{main-text-thm-ULA}. The following part establishes the global error bound with obtaining a $\frac{1}{2}\min\{c(p_t^*), c(q_t^*)\}T^{-2J}$-accurate sub-problem solution at each step along ULA.
\begin{theorem}\label{main-text-global-convergence}
    Let $\epsilon$ be the desired accuracy. Under Assumptions \ref{ass:a1}, \ref{ass:a2} and \ref{ass:a4}, if we run Langevin algorithm with step size $\iota=\Theta\left(\min\left\{\frac{\lambda_1}{\lambda_2},\frac{\lambda_1^3}{\lambda_2^3}\right\}\frac{\epsilon^2}{(\max\{m,n\})^2\exp{(30/\lambda_2)}}\right)$ for $T_t=\tilde{\Theta}\left(\iota^{-1}\lambda_1^{-1}[\lambda_2\exp{(30/\lambda_2)}\log(\epsilon^{-1})]\right)$ iterations on the inner loop, then we can achieve an $\epsilon$-accurate Max-Min gap solution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$ with probability at least $1-\delta$ when running Algorithm \ref{alg:algorithm} for iterations $T$
    and sample size $M$ with
    $$T=\Tilde{\Theta}\left(\max\left\{\log\left(\frac{\lambda_2}{\epsilon(1-\mu)}\right)/\log(\mu^{-1}),\, \, \epsilon^{-1/J}\right\}\right)$$ 
    $$M = \Tilde{\Theta}\left(\epsilon^{-2}\left[\log(\frac{T}{{\delta}})+d\log\left(1+\sqrt{\frac{\lambda_2}{\lambda_1}}\epsilon^{-1}\right)\right]\right)$$
    on the outer loop, where $d = \max\{m,n\}$ is the dimension.
\end{theorem}
Note that $\mu\leq (1+\lambda_2)^{-1}$ by Eq.~\eqref{parameter-setting}. Then we obtain the computation time $T=\Tilde{\Theta}(\max\{\log(\epsilon^{-1})/\log(1+\lambda_2)),\, \epsilon^{-1/J}\})$ if $\lambda_2 \rightarrow 0$, which indicates the limiting behavior of vanishing entropy regularizer.
Moreover, according to Eq.~\eqref{Max-Min-gap-control-entropy}, we can also control $\mathrm{KL}(\Bar{p}\|\Bar{p}^*)$ and $\mathrm{KL}(\Bar{q}\|\Bar{q}^*)$ similarly (Corollary \ref{col:kl_conv}).

% \begin{corollary}
%     Under Assumption \ref{ass:a1} and a fixed positive integer $J$, if we run the Langevin dynamic \eqref{Langevin-dynamic-q} and \eqref{Langevin-dynamic-p} with time $t'=\Tilde{\Theta}(\frac{J\log(T)}{\alpha})$ on the inner loop, and Algorithm \ref{alg:algorithm} for $T=\Tilde{\Theta}(\min\{\log(1/\epsilon), (1/\epsilon)^{1/J}\})$ iterations on the outer loop, then we can obtain an $\epsilon$-Max-Min-gap solution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$. Moreover, an $\epsilon$-KL-divergence-accurate solution: $\mathrm{KL}(q_*||q)+\mathrm{KL}(p_*||p)\leq\epsilon$ of objective \eqref{eq:problem_particle} can be achieved as well.
% \end{corollary}\congfang{theorem???}
% \begin{corollary}
%     Assume the parameter spaces of strategies $\cX$ and $\cY$ are compact Riemannian manifolds without boundary of dimension $m$, $n$ embedded in $\mathbb{R}^m$, $\mathbb{R}^n$ respectively and Assumptions \ref{ass:a1}, \ref{ass:a2} and \ref{ass:a3} hold. We can obtain an $\epsilon$-Max-Min-gap solution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$ and an $\epsilon$-KL-divergence-accurate solution: $\mathrm{KL}(q_*||q)+\mathrm{KL}(p_*||p)\leq\epsilon$ of objective \eqref{eq:problem_particle} with running Algorithm \ref{alg:algorithm} for $T=\Tilde{\Theta}(\min\{\log(1/\epsilon), (1/\epsilon)^{1/J}\})$ iterations on the outer loop, and the ULA with step size $\sigma_t=\Theta\left(\min\left\{c_0\min\{\alpha, c_1\}, \frac{1}{\hat{C}_1^2\hat{C}_0^2}T^{-2J}\right\}\right)$ for $T_t=\Tilde{\Theta}\left(\frac{2J\log(T)}{\alpha\sigma_t}\right)$ on the inner loop where $J$ is a fixed positive integer.
% \end{corollary}
% Th\epsilondefinitions of $\nabla_x h^{(t)}(x)$ and $\nabla_y g^{(t)}(y)$ in Algorithm \ref{alg:algorithm} satisfy
% \begin{align}
%     \nabla_yh^{(t)}(y)=&\sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)\frac{1}{\lambda_2+\tau_i}\left\{\mu_{i}\right.
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \mathbb{E}_{\tilde{X}^{(i-2)}}[\nabla_y f(\cdot,y)]-(1+\mu_i)
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \left.\mathbb{E}_{\tilde{X}^{(i-1)}}[\nabla_y f(\cdot, y)]\right\}+(2+\delta)
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \,  \sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)\frac{1}{\lambda_2+\tau_i}\|y\|^\delta y
%     \notag
%     \\
%     &\, \, \, \, +\frac{2\lambda_1}{\lambda_2}\left(\prod_{l=1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)y,
%     \notag
%     \\
%     \nabla_x g^{(t)}(x)=&\sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)\frac{1}{\lambda_2+\eta_i}
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \, \mathbb{E}_{\tilde{Y}^{(i)}}[\nabla_x f(x,\cdot)]+(2+\delta)\notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \, \sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)\frac{1}{\lambda_2+\eta_i}\|x\|^\delta x
%     \notag
%     \\
%     &\, \, \, \, +\frac{2\lambda_1}{\lambda_2}\left(\prod_{l=1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)x.\notag
% \end{align}

==> parts/method_neurips.tex <==

\section{Preliminary}\label{sec:preli}

\noindent\textbf{Notation.} We use lower-case letters $x, y$ to denote
vectors. For function $f:\RR^d\rightarrow\RR$, 
$\nabla f(\cdot)$ and $\nabla^2 f(\cdot)$ denote its gradient and  Hessian matrix, respectively. 
For function $f:\RR^d\rightarrow\RR^d$, $\nabla f(\cdot)$ denotes the
Jacobian matrix.
For multivariate function $f(x,y)$, $\nabla_x$, $\nabla_y$ denote the gradient over $x$, $y$.
Notation $\Vert\cdot\Vert$ denotes 2-norm for both vector and matrix. 
The continuous probability measures in this paper are considered to be absolutely continuous by default with respect to the Lebesgue measure, which induces density function $p$ and $q$. The smoothness is guaranteed by Gaussian initialization and Gaussian smoothing during the updates.
For twice differentiable function $f:\RR^d\rightarrow\RR$, we say that $f$ is $L_0$-Lipschitz if  $|f(x)-f(y)|\leq L_0 \Vert x-y\Vert$ for any $x,y\in\RR^d$; we say that $f$ has $L_1$-Lipschitz gradient if $\|\nabla f(x)-\nabla f(y)\|\leq L_1 \Vert x-y\Vert$ for any $x,y\in\RR^d$. For any a topological space  %we say that $f$ has $L_2$-Lipschitz Hessian if $\|\nabla^2 f(x)-\nabla^2 f(y)\|\leq L_2 \Vert x-y\Vert$ for any $x,y\in\RR^d$
$\mathcal{X}$, $\mathcal{P}(\mathcal{X})$ denotes set of probability measures on $\cX$ and 
$\mathcal{P}_2(\mathcal{X})$ denotes the set of probability measures with bounded second moments.
For density $p$, we define $\cE(p)=\mathbb{E}_p[\log(p)]$, $\mathrm{KL}(p\|q)=\mathbb{E}_p[\log (p/q)]$. For the generalized density for particles, we use Dirac delta distribution $\dirac_{x}$ to represent the Dirac delta distribution at $x$, $\dirac_{\{x_1,\cdots,x_n\}} = n^{-1}\sum_{i=1}^n\dirac_{x_i}$.



%%where $R(\cdot)$ is a density regularizer.
\noindent\textbf{Problem Setup.}
Assume that the min-max problem is defined on the space $\cX \times \cY$ with a function $f: \cX \times \cY\rightarrow \RR$. 
We consider the bounded case. For simplicity without loss of generality, the
domain $\cX \times \cY$ is the 
Euclidean space $\RR^m\times\RR^n$ and the co-domain of $f$  is a bounded interval $[-1,1]$. In our work, we consider the regularized minimax problem defined in Eq.~\eqref{eq:problem_particle}. We set 
\begin{equation}\label{eq:relative_reg}
\cR(p(x))=\EE_{p(x)}\left[\lambda_1\|x\|^{2}+\lambda_2\log(p(x))\right] 
\end{equation}
where $\lambda_1,\lambda_2>0$ are constants to determine the regularization scaling as well as the variance of the prior.
We use $\cL(p,q)$ to denote $\EE_{p(x)} \EE_{q(y)} f(x,y)  + \cR(p) - \cR(q)$.
%Recall that a pure Nash equilibrium denotes a pair of strategies $(x,y)\in \cX \times \cY$ such that for all $(x',y')\in \cX \times \cY$, $f(x,y') \leq f(x,y)\leq f(x',y)$.  Similarly, 
The mixed Nash equilibrium denotes a distribution pair $(p_*,q_*)$ such that for all $(p,q)\in \cP(\cX )\times \cP(\cY)$, $\cL(p_*,q) \leq \cL(p_*,q_*)\leq \cL(p,q_*)$. Therefore, for any distribution pair $(\bar{p},\bar{q})$, the duality gap $\max\limits_{q\in\cP(\cY)}\mathcal{L}(\bar{p},q)-\min\limits_{p\in\cP(\cX)}\mathcal{L}(p,\bar{q})$ forms the basis for a standard optimality criterion. Formally, we define as below.
\begin{definition}[$\epsilon$-MNE]
    A distribution pair $(\bar{p},\bar{q})$ is an $\epsilon$-mixed Nash equilibrium ($\epsilon$-MNE) of function $\mathcal{L}(\cdot,\cdot)$ if $\max\limits_{q\in\cP(\cY)}\mathcal{L}(\bar{p},q)-\min\limits_{p\in\cP(\cX)}\mathcal{L}(p,\bar{q})\leq \epsilon$. If $\epsilon=0$, $(\bar{p},\bar{q})$ is a mixed Nash equilibrium.
\end{definition}


Assumptions are listed below.
\begin{enumerate}[label={\textbf{[A$_\text{\arabic*}$]}}]
    \item There exists $L_0$ such that $f$ is $L_0$-Lipschitz.\label{ass:a1}
    \item $f$ has $L_1$-Lipschitz gradient.\label{ass:a2}
 \item For any $x,y\in \cX\times\cY$, $| f(x,y)|\leq 1$.\label{ass:a4}
\end{enumerate}

We consider the bounded function with growth regularities. The bound of $|f|$ is chosen as 1 for notation simplicity.
 \ref{ass:a1}, \ref{ass:a2} regularize the growth of $f$, $\nabla f$ respectively and the definition of  Lipschitz continuity was introduced in \textbf{Notation}. Our setting is general given the above assumptions.
%$\nabla^2 f$


\noindent\textbf{Primal-Dual Algorithms for Min-Max Optimization.}
primal-dual method is a classical approach to solve saddle point problems \citep{nemirovski2004prox,he2017algorithmic,lan2020first,bredies2015preconditioned,luke2018globally}. For example, consider the min-max problem
\begin{align}\label{saddle-point-problem}
    \min_{x\in \cX}\max_{y\in \cY}\left\{f(x)+\langle Ax,y\rangle-g(y)\right\},
\end{align}
where $A\in\mathbb{R}^{m\times n}$ denotes a linear mapping, and $f:\cX\rightarrow \mathbb{R}$ and $g:\cY\rightarrow \mathbb{R}$ are two convex functions. General optimization problems with linear constraints: $\min\limits_{x\in\cX}\{f(x):Ax=b \}$ \congfang{can be transformed to}
%is a special case covered by
Eq.~\eqref{saddle-point-problem}. The proximal primal-dual algorithm updates $x_t$ and $y_t$ according to
\begin{align}
    \Tilde{x}_t=&x_{t-1}+\mu_t(x_{t-1}-x_{t-2}),
    \\
    y_t=&\arg\min\limits_{y\in\cY}\langle-A\Tilde{x}_t,y\rangle+g(y)+\tau_t W(y_{t-1},y),
    \\
    x_t=&\arg\min\limits_{x\in\cX}\langle y_t,Ax\rangle+f(x)+\eta_t V(x_{t-1}, x),
\end{align}
under a finite dimension condition with $W$ and $V$ representing Bregman's distances on $\cY$ and $\cX$, respectively. Moreover, $\{\tau_t\}, \{\eta_t\}, \{\gamma_t\}$ are algorithmic parameters to be specified.  The
Bregman divergence is particularly important for other Riemannian structures.
In probability space, the Bregman divergence is usually chosen as KL divergence or Wasserstein distance.

%Specially, the accelerated gradient descent method in can be viewed asa special case of the above primal-dual method \cite{lan2020first}.
 



\noindent\textbf{Unadjusted Langevin Algorithm.} We introduce 
\emph{Unadjusted Langevin Algorithm (ULA)}
to solve the mirror steps. Isoperimetry inequalities shall be introduced to make each step well-posed.


\begin{definition} \citep{gross1975logarithmic}
We say that $p$ satisfies log-Sobolev inequality (LSI) with a constant $\alpha>0$, if $
    \mathbb{E}_{p}[g^2\log(g^2)]-\mathbb{E}_{p}[g^2]\log\mathbb{E}_{p}[g^2]\leq\frac{2}{\alpha}\mathbb{E}_{p}[\|\nabla g\|^2]
$
for all differentiable $g$ with 
 $\mathbb{E}_{p}[g^2]<\infty$. When $g = \sqrt{p/q}$, we have 
$
\mathrm{KL}(p\Vert q) \leq \frac{1}{2\alpha} \EE_p \left\Vert \nabla \log \frac{p}{q}\right\Vert^2.
$
\end{definition}

Assume we aim to sample from a smooth target probability density $p\propto e^{-f(x)}$ where $f(x)$ has $L_1$-Lipschitz gradient and satisfies a smoothness condition. The ULA with step size $\eta>0$ is the discrete-time algorithm
$
    x_{s+1}=x_s-\eta\nabla f(x_s)+\sqrt{2\eta}\zeta_s,
$
where $s=0,\cdots,T$ for some positive integer $T$; $x_0$ is given as an initialization;  
$\zeta_s\sim\mathcal{N}(0,I)$ is an isotropic Gaussian noise. Moreover, if $p$ satisfies LSI, we can guarantee that $\rho_s$ converge to 
$p_\epsilon$ with a linear convergence rate in KL divergence under fixed step size, where
$\rho_s$ is the density of  $x_s$ along ULA at step-$s$, and $p_\epsilon$ is a biased stationary distribution.
The $\text{KL}(\rho_s\|p)$ along ULA would also converge to $\cO(\epsilon)$. 
Since it is equivalent with gradient descent with additional Gaussian noise, it is easy to implement in practice. 
Moreover, 
the asymptotic bias along ULA in KL divergence $\text{KL}(p_\epsilon\|p)$  can be reduced with a sufficiently small step size.
The  easy-to-implement property and the arbitrarily small bias make it a popular in sampling literature. Thus, we choose it to solve our sub-problems.

%As $\epsilon\rightarrow 0$, ULA recovers the Langevin dynamics in continuous-time. 
%to 
%with linear rate
%with the following error bound \citep{vempala2019rapid}\begin{align}    \text{KL}(\rho_s\|p)\leq e^{-\alpha\epsilon s}\text{KL}(\rho_0\|p)+\frac{8\epsilon mL_1^2}{\alpha},\end{align}

%where $\rho_s$ is the probability density of random variable $x_s$ that evolves ULA at step-$s$; $m$ is the dimension; $\epsilon$ denotes the step size.

\iffalse
The ULA with step size $\epsilon>0$ is the discrete-time algorithm
\begin{align}
    x_{s+1}=x_s-\epsilon\nabla f(x_s)+\sqrt{2\epsilon}\zeta_s,
\end{align}
where $s=0,\cdots,T$ for some positive integer $T$; $x_0$ is given as initialization;  
$\zeta_s\sim\mathcal{N}(0,I_m)$ is an isotropic Gaussian noise drawn in $\mathbb{R}^m$. Specifically, we can write $s$-th step of ULA \eqref{Langevin-dynamic-main-text} as the output at time $\epsilon$ of the stochastic differential equation
\begin{align}\label{eq:disc}
    dx_{s+t}=- \epsilon\nabla f(x_{s})dt+\sqrt{2\epsilon}dW_t^m,\quad t\in[0,1]
\end{align}
where  $\epsilon$ is the step size and $W_t^m$ is the standard Brownian motion in $\mathbb{R}^m$ starting at $W_0^m=0$. 
Eq.~\eqref{eq:disc} represents the discretized Langevin dynamics.


The continuous version evolves  as following
\begin{align}\label{Langevin-dynamic-main-text}
    dx_{s+t}=-\epsilon\nabla f(x_{s+t})dt+\sqrt{2\epsilon}dW_t^m, \quad t\in[0,1]
\end{align}
where $\epsilon$ is the step size and $W_t^m$ is the standard Brownian motion in $\mathbb{R}^m$ starting at $W_0^m=0$. 
\fi
%$\nabla f(x_{s+t})$ is a time-dependent drift force in each interval. 






\begin{algorithm*}[t]
\caption{Particle-based Primal-Dual Algorithm for Mixed Nash Equilibrium} \label{alg:algorithm}
\hspace*{0.02in} {\bf Input:} 
 number of outer iterations $T$, outer-loop learning rates $\{\eta_t\}_{t=1}^T$ and $\{\tau_t\}_{t=1}^T$,  outer-loop hyper-parameters $\{\mu_t\}_{t=1}^T$; number of inner iterations $\{T_t\}_{t=1}^T$, inner-loop learning rates $\{\iota_t\}_{t=1}^T$, 
 number of particles $M$
 \\
\hspace*{0.02in} {\bf Output:} estimated equilibrium   
$(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}})$

\begin{algorithmic} 
\STATE Initialize $\{\Tilde{x}_r^{(0)}\}_{r=0}^M\sim p_0(x)\propto\exp\left\{-\frac{\lambda_1}{\lambda_2}\|x\|^2\right\},\ \{\Tilde{y}_r^{(0)}\}_{r=0}^M\sim q_0(y)\propto\exp\left\{-\frac{\lambda_1}{\lambda_2}\|y\|^2\right\}.$ 

Assign $(\tilde{X}^{(-1)},\tilde{Y}^{(-1)})=(\tilde{X}^{(0)},\tilde{Y}^{(0)})\leftarrow\left(\{\Tilde{x}_r^{(0)}\}_{r=1}^M, \{\Tilde{y}_r^{(0)}\}_{r=1}^M\right)$.

Assign $h^{(0)}(y) = \frac{\lambda_1}{\lambda_2}\|y\|^2 $, $g^{(0)}(x) = \frac{\lambda_1}{\lambda_2}\|x\|^2 $.
\FOR{$t=0$ to $T-1$}
    \STATE Initialize $(X^{(0)},Y^{(0)})\sim p_0(x)\times q_0(y)$.
    \STATE Update $
    h^{(t+1)}(y) 
    =\frac{1} {\lambda_2+\tau_{t+1}}\left\{\hat{\phi}_{t+1}(y)
+\lambda_1\|y\|^{2}+\tau_{t+1}h^{(t)}(y)\right\}.
    $
    \FOR{$k=0$ to $T_t$, $r=0$ to $M$}
        %\STATE for $r\in\{1,2,\cdots,M\}$
        %\STATE $\nabla_y h^{(t+1)}(y)=\frac{1} {\lambda_2+\tau_{t+1}}\left\{\int \nabla_y f(x, y)[\mu_{t+1}p_{t-1}-(1+\mu_{t+1})p_{t}](x)dx+(2)\lambda_1\|y\|^{\delta}y\right\}+\frac{\tau_{t+1}}{\lambda_2+\tau_{t+1}}\nabla_y h^{(t)}(y)$
        \STATE Run noisy GD 
        $y_r^{(k+1)}\leftarrow y_r^{(k)}-\iota_t\nabla_y h^{(t+1)}(y_r^{(k)})+\sqrt{2\iota_t}\xi_r^{(k)}$, where $\xi_r^{(k)}\sim\mathcal{N}(0, I_{n})$.
    \ENDFOR
    \STATE Assign $\Tilde{Y}^{(t+1)}\leftarrow Y^{(T_t+1)}$.
    \STATE Update $
    g^{(t+1)}(x)
    =\frac{1} {\lambda_2+\eta_{t+1}}\left\{\hat{\psi}_{t+1}(x)+\lambda_1\|x\|^{2}+\eta_{t+1} g^{(t)}(x)\right\}.
    $
    
    \FOR{$k=0$ to $T_t$, $r=0$ to $M$}
        %\STATE  for $r\in\{1,2,\cdots,M\}$
        %\STATE $\nabla_x g^{(t+1)}(x)=\frac{1} {\lambda_2+\eta_t}\left\{\int\nabla_x f(x,y)q_{t+1}(y)dy+(2)\lambda_1\|x\|^{\delta}x\right\}+\frac{\eta_t}{\lambda_2+\eta_t}\nabla_x g^{(t)}(x).$
        \STATE Run noisy GD $x_r^{(k+1)}\leftarrow x_r^{(k)}-\iota_t\nabla_x g^{(t+1)}(x_r^{(k)})+\sqrt{2\iota_t}\zeta_r^{(k)}$, where $\zeta_r^{(k)}\sim\mathcal{N}(0, I_{m})$.
    \ENDFOR
    \STATE Assign $\Tilde{X}^{(t+1)}\leftarrow X^{(T_t+1)}$.
    
\ENDFOR 

\textbf{Option I:} $
(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}}) \leftarrow 
(\frac{1}{M}\dirac_{\Tilde{X}^{(T)}},\frac{1}{M}\dirac_{\Tilde{Y}^{(T)}})$.

\textbf{Option II:} Randomly pick up $t\in\{1,\cdots,T\}$ following $\mathbb{P}[t]=\frac{\mu_t}{\sum_{t=1}^T\mu_t}$ as $(\frac{1}{M}\dirac_{\hat{X}},\frac{1}{M}\dirac_{\hat{Y}})$.
\end{algorithmic}
\end{algorithm*}



\section{Particle-based Primal-Dual Algorithm}
We propose Particle-based Primal-Dual Algorithm (PAPAL) to solve the regularized minimax problem Eq.~\eqref{eq:problem_particle} by applying Unadjusted Langevin Algorithm (ULA) to Mirror-Prox Primal-Dual method.
%\congfang{???} In particular, we introduce the Langevin dynamics convergence of our method to illustrate the algorithmic intuition and develop the convergence analysis for infinite-dimension mirror-prox on probability measures using the bound on density ratio in sub-problem.\congfang{???}

As an optimization algorithm on the space of  continuous probability measures, our proposed PAPAL (Algorithm \ref{alg:algorithm}) consists of two components: inner loop and outer loop. Specifically,
our outer loop extends the classical primal-dual scheme (Sec. \ref{sec:preli}) to infinite dimensional optimization problems. Each outer step can be rewriten as a sampling task for Gibbs distribution. We perform ULA as the inner loop to approximate a proximal Gibbs distribution, which is applied to the outer loop optimization to converge to the $\epsilon$-mixed Nash equilibrium distributions $\Bar{p}$ and $\Bar{q}$. We will provide the motivation of our algorithm from an optimization view.

% In the following parts, we will provide the interpretation and motivation of our algorithm thoroughly.

\noindent\textbf{Exact Primal-Dual Method.}%\label{sec:pd} 
We construct the target density of $p^*_t$ and $q^*_t$ for each iteration. Particularly, given $\hat{p}_{-1}$, $\hat{p}_0$, and $\hat{q}_0$,
$q_t^*(y)$ and $p_t^*(x)$ satisfy the following recursive condition,
    \begin{align}              
q_t^*:=&\argmin_{q\in\cP(\cY)}\mathbb{E}_q[\hat{\phi}_t(y)]+\cR(q) +
        \tau_t \mathrm{KL}(q\|q_{t-1}^*), \label{minimizer-q}
        \\ p_t^*:=&\argmin_{p\in\cP(\cX)}\mathbb{E}_p[\hat{\psi}_t(x)]+\cR(p)
        +\eta_t \mathrm{KL}(p\|p_{t-1}^*), \label{minimizer-p}
    \end{align}
    where $\hat{\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{\hat{p}_{t-1}}[f(\cdot,y)]+\mu_t\mathbb{E}_{\hat{p}_{t-2}}[f(\cdot,y)]$, and $\hat{\psi}_t(x)=\mathbb{E}_{\hat{q}_t}[f(x,\cdot)]$. 

    If $\hat{q}_t = q_t^*$, $\hat{p}_t = p_t^*$, Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} perform exact primal-dual method in continuous probability space, with KL divergence as the Bregman divergence. However,
    there two gaps for the aforementioned updates: 
    (1) the forms of $q_{t-1}^*$ and $p_{t-1}^*$ are not explicit in Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p};
    (2) the exact solutions for $\hat{q}_t$ and $\hat{p}_t$ are not tractable. To adapt to particle approximation, it is necessary to adjust the structure of the inner product in primal-dual iteration Eq.~\eqref{minimizer-q}, Eq.~\eqref{minimizer-p} appropriately, i.e, converting $(q_{t-1}^*,p_{t-1}^*)$ to a feasible form and approximating the optimal $(q_t^*,p_t^*)$..
    % Thus, it is necessary to derive to feasible form of $(q_{t-1}^*,p_{t-1}^*)$ and approximate the optimal $(q_t^*,p_t^*)$.

    
    %\noindent\textbf{Remark.} We would like to distinguish 
    %\hanze{\\TBA \\ more clear clarification about $p^*_t$, $p_t$, and $\hat{p}_t$\\(Monte Carlo)}

    %the computation and update on particles should still be adapted. 

\noindent\textbf{Recursive Energy Function.}
In this part, we would discuss the feasibility of the proposed updates.
%Importantly, the loss function Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} include $q_*^{t-1}$ and $p_*^{t-1}$ term, which are not explicit in an algorithm.
 The following Lemma provides us insight to obtain the explicit form of $q_*^{t-1}$ and $p_*^{t-1}$ in  Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} recursively, which can be implemented in an algorithm.


\begin{lemma}\label{lemma:optimal-KL-prox}
    Let $\lambda>0$ be a positive real number and $\tilde{l}(\theta), l(\theta)$ be bounded continuous functions. Consider a probability density $\Bar{p}(\theta)\propto\exp\left(-\tilde{l}(\theta)\right)$, then $p(\theta)\propto\exp\left(-\frac{1}{\lambda+\tau}l(\theta)-\frac{\tau}{\lambda+\tau}\tilde{l}(\theta)\right)$ is an optimal solution to the following problem  
    \begin{align}
        \min\limits_{p\in\mathcal{P}(\Theta)}\{\mathbb{E}_{p}[l(\theta)]+\lambda \cE(p)+\tau \mathrm{KL}(p\|\Bar{p})\}.
    \end{align}
\end{lemma}

Once we obtained two approximate distributions
$\hat{p}_i(y)$ and $\hat{p}_i(x)$, Lemma \ref{lemma:optimal-KL-prox} indicates that if $p_{t-1}^*$ and $q_{t-1}^*$ are proximal Gibbs distribution
with explicit form. 
Then, $p_t^*$ and $q_t^*$ have the similar expression as well. Therefore, we denote 
    \begin{align*}
    h^{(t)}(y) 
    =\frac{\hat{\phi}_t(y)
+\lambda_1\|y\|^{2}+\tau_th^{(t-1)}(y)} {\lambda_2+\tau_t},\ 
    g^{(t)}(x)
    =\frac{\hat{\psi}_t(x)+\lambda_1\|x\|^{2}+\eta_t g^{(t-1)}(x)} {\lambda_2+\eta_t}.
    \end{align*}

    % $h^{(t)}(y):=\sum_{i=1}^t a_{i}^t\left\{\mu_{i}\mathbb{E}_{p_{i-2}}[f(\cdot,y)]-\right.\\
    % \left.(1+\mu_i)\mathbb{E}_{p_{i-1}}[f(\cdot, y)]\right\}+\sum_{i=1}^t
    % a_{i}^t\|y\|^{2}+\frac{a_{1}^t\tau_1}{\lambda_2}\|y\|^2$ and $a_{i}^t=\frac{\lambda_1}{\lambda_2+\tau_i}\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}$
    
    % $g^{(t)}(x):=\sum_{i=1}^t b_{i}^t\mathbb{E}_{q_i}[f(x,\cdot)]+\sum_{i=1}^t b_{i}^t\|x\|^{2}+\frac{b_{1}^t \eta_1 }{\lambda_2}
    % \|x\|^2$ and $b_{i}^t=\frac{\lambda_1}{\lambda_2+\eta_i}\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}$
    
    which consist of the Gibbs potential on $\mathcal{P}_2(\mathcal{Y})$ and $\mathcal{P}_2(\mathcal{X})$ after $t-1$ iterations. Thus, at each step-$t$, our objective probability densities can be written as 
    \begin{align}
        q_t^*(y)=\frac{\exp\left(-h^{(t)}(y)\right)}{Z_{t,1}},\, \, \, \, p_t^*(x)=\frac{\exp\left(-g^{(t)}(x)\right)}{Z_{t,2}},\notag
    \end{align}
    where $Z_{t,1}$ and $Z_{t,2}$ are normalizing constants. 
%(the approximate probability densities we obtain are $q_t(y)$ and $p_t(x)$)
%\subsection{Particle Approximation}

\noindent\textbf{Inexact Solver and Particle Approximation.} For each step-$t$, the ideal case ($\hat{q}_t = q_t^*$, $\hat{p}_t = p_t^*$) is not tractable in the algorithm. Since there is not closed form to compute Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}.
Fortunately, the optimization of random variables can be approximately done given the log density. ULA is a widely algorithm to approximate the target distribution. After several steps, 
$(q_t,p_t)$ can be obtained to approximate $(q^*_t,p^*_t)$. Thus, $\hat{q}_t = q_t$ and $\hat{p}_t = p_t$ lead to an approximated algorithm given Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}. Nonetheless, the realization of $(q_t,p_t)$ pair can only be executed a finite number of times. Thus, the $(q_t,p_t)$ pair in an algorithm should be a pair of particle sample sets, which is denoted as $(\hat{q}_t,\hat{p}_t)$.
Specifically, the full procedure can be done as follows.

We initialize a set of particles and duplicate it  $\left\{x_r^{(-1)},y_r^{(-1)}\right\}_{r=1}^M =\left\{x_r^{(0)},y_r^{(0)}\right\}_{r=1}^M
$. 
For each step, we optimize particles in $\cY$ using ULA. At the $k$-th inner step, the gradient is estimated by $x_r^{(k-1)}$, $x_r^{(k-2)}$ and $\nabla_y h^{(t)}(y_r^{(k)})$.
%we run ULA to optimize the particles in $\cY$,  where the gradient at the $k$-th inner step is given by $\nabla_y h^{(t)}(y_r^{(k)})$ estimated by $x_r^{(k-1)}$ and $x_r^{(k-2)}$.
Similarly, we repeat the process for $\cX$, and we estimate the gradient using $y_r^{(k-1)}$ and $\nabla_y g^{(t)}(x_r^{(k)})$.
% Then, we execute the same process as above starting from the prior where the gradient at the $k$-th inner step is given by $\nabla_y g^{(t)}(x_r^{(k)})$ estimated by $y_r^{(k-1)}$. 
We prioritize approximating probability density $q_t(y)$ (or $\hat{q}_t(y)$), because at step $t$ of primal-dual update on $\cP_2(\cX)$, we need to use the latest value of $q_t$ as an input.
% The reason why we run the Langevin algorithm on $\mathcal{P}_2(\mathcal{Y})$ firstly is that the approximate probability density $q_t(y)$ (or $\hat{q}_t(y)$) is necessary for the $t$-th optimization step on $\mathcal{P}_2(\mathcal{X})$.




%Another intractable term in the algorithm is the gap

\emph{Remark 1.} In the following parts, to make a clear
distinction between  $(\hat{q}_t,\hat{p}_t)$, $(q_t,p_t)$, and $(q^*_t,p^*_t)$, we reiterate the definition here: we initialize $(\hat{q}_{-1},\hat{p}_{-1})=(\hat{q}_0,\hat{p}_0)$ from the prior distribution. From $t=1$ to $t=T$, $(q^*_t,p^*_t)$ is the exact solution from Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}; $(q_t,p_t)$ is the ULA approximation of $(q^*_t,p^*_t)$;  $(\hat{q}_t,\hat{p}_t)$ is the realization of $(q_t,p_t)$ with $M$ samples (mixture of dirac delta distributions). All the densities above can be defined by recursion.

\emph{Remark 2.} Other sampling algorithms can be implemented as the inexact solver, such as Hamiltonian Monte Carlo \citep{duane1987hybrid,neal2011mcmc}, Metropolis-adjusted Langevin algorithm  \citep{rossky1978brownian,grenander1994representations}.
We use ULA here for demonstration and simplicity. More sophisticated solvers can usually improve the convergence rate.




\noindent\textbf{Optimization View of PAPAL.} 
In this part, we explain the algorithmic intuition behind PAPAL from an optimization perspective. Recall that Algorithm \ref{alg:algorithm} iteratively updates the particles, $\hat{q}_t$ and $\hat{p}_t$, which approximate the minimizers of the linearized potentials, presented in Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p}. 
If Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} degenerate to finite dimension, we obtain the classical primal-dual algorithm, as proposed by \cite{nemirovski2004prox}. Under this condition, we can easily derive the total complexity by finding $q_t^*$ and $p_t^*$ with negligible error.
% It is obvious that we can find $q_t^*$ and $p_t^*$ with negligible error under finite dimension condition which implies the total complexity would be derived easily. 
However, relying on Langevin algorithm to solve sub-problems in infinite dimensions poses three challenges: (1)  expressing the optimal density function forms in Eq.~\eqref{minimizer-q} and Eq.~\eqref{minimizer-p} explicitly; (2) analyzing the outer loop with the bounded KL error induced by ULA at each step-$t$; (3) controlling the error induced by finite particles at each step $t$.



The first issue may be resolved by employing forward recursion of $(q_{t-1}^*,p_{t-1}^*)$ and Lemma \ref{lemma:optimal-KL-prox}, which combining the approximated solutions $\left\{(\hat{q}_k, \hat{p}_k)\right\}_{k=-1}^{t-1}$.
To further limit the error between approximate densities and precise densities in each iteration of the primal-dual method, we introduce the LSI condition \citep{gross1975logarithmic},  which ensures the swift convergence of sampling algorithms, such as ULA. Therefore, we incorporate the regularizer that includes a $\|\cdot\|^{2}$ term with coefficient $\lambda_1$ ($\lambda_1$ may be any positive number) to warrant that $q_t^*$ and $p_t^*$ fulfill the LSI condition.
%Therefore, we add $\|\cdot\|^{2}$ term with coefficient $\lambda_1$, ($\lambda_1$ can be an arbitrary positive number) to the regularizer which guarantee that $q_t^*$ and $p_t^*$ satisfy the LSI condition. 
We approximate the actual expectation using finite particles $\hat{\phi}_t$ and $\hat{\psi}_t$. Specifically, $\hat{\phi}_t$ approximates ${\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{{p}_{t-1}}[f(\cdot,y)]+\mu_t\mathbb{E}_{{p}_{t-2}}[f(\cdot,y)]$, while $\hat{\psi}_t$ approximates $ {\psi}_t(x)=\mathbb{E}_{{q}_t}[f(x,\cdot)]$. Concentration techniques will be applied to ensure that the gap between $(\hat{\phi}_t,\hat{\psi}_t)$ and $({\phi}_t,{\psi}_t)$ is regulated.
% Finally, the finite particle $\hat{\phi}_t$ and $\hat{\psi}_t$ approximate the true expectation 
% ${\phi}_t(y)=-(1+\mu_t)\mathbb{E}_{{p}_{t-1}}[f(\cdot,y)]+\mu_t\mathbb{E}_{{p}_{t-2}}[f(\cdot,y)]$, and
% $ {\psi}_t(x)=\mathbb{E}_{{q}_t}[f(x,\cdot)]$. The gap between $(\hat{\phi}_t,\hat{\psi}_t)$ and $({\phi}_t,{\psi}_t)$ shall be controlled by concentration techniques.


To sum up, we connect bilinear forms $\langle Ax,y\rangle$ under finite dimension and $\EE_{p(x)}\EE_{q(y)}f(x,y)$ under infinite dimension by the proximal Gibbs distribution. Moreover, the estimation of both sub-problem error and finite sample error is applied for global convergence analysis of our particle-based algorithm. As a result, PAPAL can be interpreted as a finite-particle approximation of a primal-dual method. PAPAL combines the primal-dual method's efficient convergence in the outer loop, and the KL error bound of ULA under LSI condition in the inner loop. An essential advantage of our algorithm is that the loss functional can be estimated with polynomial finite particles, making it is possible to implement.
Algorithm \ref{alg:algorithm} outlines the full procedure. We have presented some empirical results in the Appendix.
%\congfang{moderate number of particles???}


\section{Convergence Analysis}
In this section,  we present quantitative global convergence for PAPAL. We begin by providing the finite sample error bound. Then, we introduce the outer loop settings and conclude the properties of the updates. By assuming the approximate optimality of the inner loop iterations, the error bound of the outer loop can be obtained.
Then, we discuss the convergence rate of the inner loop iterations, which is the KL convergence of ULA algorithm. Finally, we combine the outer loop and the inner loop to discuss the total complexity of PAPAL. We provide the global convergence results of our main theorem.

\noindent\textbf{Finite Sample Error.} We concentrate on probability sets $\cQ_{\cX}$ and $\cQ_{\cY}$ as follows
 \begin{align*}
     &\cQ_{\cX}:=\left\{p(x)\propto e^{-l_1(x)-\frac{\lambda_1}{\lambda_2}\|x\|^2}; \|l_1\|_\infty\leq \frac{C}{\lambda_2}\right\},\ \cQ_{\cY}:=\left\{q(y)\propto e^{-l_2(y)-\frac{\lambda_1}{\lambda_2}\|y\|^2};\|l_2\|_\infty\leq \frac{C}{\lambda_2}\right\},
 \end{align*}
 for a fixed positive constant $C$. The form of the objective function in Eq.~\eqref{eq:problem_particle} indicates that only the discretization error on the linear term needs to be bounded. In order to bound the discretization error between $\hat{p}_t$ and $p_t$ ($\hat{q}_t$ and $q_t$) at step $t$, we use the following lemma (see proof in Appendix \ref{discre}).
 %By the form of objective function in Eq.~\eqref{eq:problem_particle}, we just need to bound the discretization error on linear term. Therefore, we use the following lemma to bound the discretization error between $\hat{p}_t$ and $p_t$ ($\hat{q}_t$ and $q_t$) at each step-$t$ (Appendix \ref{discre}).
 \begin{lemma}\label{finite-particle-approximation}
     The errors of finite particles satisfy
     \begin{align*}
         &\mathbb{P}\left[\left|(\hat{p}_t-p_t)(x)f(x,y)q(y)dydx\right|\geq\epsilon\right]\leq\delta,\quad 
         \mathbb{P}\left[\left|(\hat{q}_t-q_t)(y)f(x,y)p(x)dxdy\right|\geq\epsilon\right]\leq\delta,
     \end{align*}
     with the required numbers of particle $M:=\mathcal{O}\left(\epsilon^{-2}\left[-\log(\delta)+d\log(1+L_0\sqrt{\lambda_2/\lambda_1}\epsilon^{-1})\right]\right)$ 
     on $\hat{p}_t(x)$ and $\hat{q}_t(y)$ for all $p(x)\in\cQ_{\cX},\, q(y)\in\cQ_{\cY}$ where $d=\max\{m,n\}$ is the dimension.
 \end{lemma}

\noindent\textbf{Outer Loop Error Bound.} 
We introduce the Max-Min gap function 
\begin{align}
    Q(\Bar{w},w):=\mathcal{L}(\Bar{p},q)-\mathcal{L}(p,\Bar{q}),
\end{align}
where $\Bar{w}:=(\Bar{p},\Bar{q})$ and $w:=(p,q)$. Note that $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)$ is equivalent to the duality gap on $(\Bar{p},\Bar{q})$, as previously mentioned.

Specially, under the expression of objective function in Eq.~\eqref{eq:problem_particle} and \eqref{eq:relative_reg}, we have
\begin{equation}\label{Max-Min-gap-control-entropy}
\max_{w}Q(\Bar{w},w)\geq\lambda_2(\mathrm{KL}(\Bar{p}\|\Bar{p}^*)+\mathrm{KL}(\Bar{q}\|\Bar{q}^*)),\ \text{s.t.} \quad\Bar{w}^*=(\Bar{p}^*,\Bar{q}^*)=\argmax_{w'}Q(\Bar{w},w')
\end{equation}
where the domain of $w,w'$ is $\cP_2(\cX)\times\cP_2(\cY)$.
According to Eq.~\eqref{Max-Min-gap-control-entropy}, the duality gap on $\Bar{w}$ can regulate the KL divergence between $\Bar{w}$ and $\Bar{w}^*$.

To capture the error of our algorithm, we assume that the KL divergence between $(q_t,p_t)$ and $(q^*_t,p^*_t)$ can be bounded by a small error, i.e.,
$\mathrm{KL}(p_t\|p_t^*)\leq\delta_{t,1},\ \mathrm{KL}(q_t\|q_t^*)\leq\delta_{t,2},$
which is guaranteed by ULA algorithm with small step sizes (Theorem \ref{main-text-thm-ULA}). We use the 
error bound quantities $\delta_{t,1}$
and $\delta_{t,2}$ to analyze the outer loop properties. The following theorem proves the general convergence properties of mirror-prox primal-dual method with an inexact solver.
 %Next, we need to control a set of quantities of error bound for $p_t$ and $q_t$ in the inner loop, 
% \begin{theorem}\label{main-text-outer-loop-thm}
% After $T$ iterations of Primal-Dual method 
% with setting $\gamma_t\mu_t=\gamma_{t-1}$,\,  $\gamma_t\tau_t\leq\gamma_{t-1}(\tau_{t-1}+\lambda_2)$,\, $\gamma_t\eta_t\leq\gamma_{t-1}(\eta_{t-1}+\lambda_2)$,\, $\tau_t\eta_{t-1}\geq\mu_t$ for any $t\geq1$ and the sub-problem errors have been bounded by $\delta_{t,1}(p),\delta_{t,1}(q);\delta_{t,2}(p),\delta_{t,2}(q)$ mentioned above, the estimation of Max-Min gap satisfies
% \begin{align}
%     &\sum_{t=1}^T\gamma_t Q(w_t,w)\notag
%     \\
%     \leq&\gamma_1\eta_1\mathrm{KL}(p\|p_0)-\gamma_T(\eta_T+\lambda_2)\mathrm{KL}(p\|p_T)\notag
%     \\
%     &+\gamma_1\tau_1\mathrm{KL}(q\|q_0)-\gamma_T\left(\tau_T+\lambda_2-\frac{1}{4\eta_T}\right)\mathrm{KL}(q\|q_T)\notag
%         \\
%         &+\sum_{t=1}^T\gamma_t\{(\tau_t+2\tau_{t+1}+\lambda_2)\left[\delta_{t,1}(q)+\delta_{t,2}(q)\right]\notag
%         \\
%         &\, \, \, \, \, \, \, \,  +(\eta_t+2\eta_{t+1}+\lambda_2)\left[\delta_{t,1}(p)+\delta_{t,2}(p)\right]\}.
% \end{align}
% \end{theorem}
\begin{theorem}\label{main-text-outer-loop-thm}
By setting parameters $\gamma_t\mu_t=\gamma_{t-1}$,\,  $\gamma_t\tau_t\leq\gamma_{t-1}(\tau_{t-1}+\lambda_2)$,\, $\gamma_t\eta_t\leq\gamma_{t-1}(\eta_{t-1}+\lambda_2)$,\, $\tau_t\eta_{t-1}\geq\mu_t,\, \mu_t\leq 1$ for any $t\geq1$ and optimizing the sub-problem with errors bounded by $\delta_{t,1}, \delta_{t,2}$ mentioned above, iterates of our method satisfies
\begin{align*}
    &\sum_{t=1}^T\gamma_t Q(w_t,w)\notag
    \leq\gamma_1\eta_1\mathrm{KL}(p\|p_0^*)-\gamma_T(\eta_T+\lambda_2)\mathrm{KL}(p\|p_T^*)
    +\gamma_1\tau_1\mathrm{KL}(q\|q_0^*)
        \\
        &+\sum_{t=1}^k\gamma_t\left[\left(\lambda_2+\frac{2\lambda_1}{\alpha_{p_t^*}}\right)\delta_{t,1}+\left(30+\frac{8\lambda_1\sigma(p_t^*)}{\sqrt{\alpha_{p_t^*}}}\right)\sqrt{\delta_{t,1}}\right]\notag
        -\gamma_T\left(\tau_T+\lambda_2-\frac{1}{4\eta_T}\right)\mathrm{KL}(q\|q_T^*)\\
&+\sum_{t=1}^k\gamma_t\left[\left(\lambda_2+\frac{2\lambda_1}{\alpha_{q_t^*}}\right)\delta_{t,2}+\left(34+\frac{8\lambda_1\sigma(q_t^*)}{\sqrt{\alpha_{q_t^*}}}\right)\sqrt{\delta_{t,2}}\right]+4\sum_{t=1}^k\gamma_t (1+\mu_t)\epsilon,
\end{align*}
for any $p\in\cQ_{\cX}, q\in\cQ_{\cY}$ with probability at least $1-{\delta}$ for sample size $M=\Tilde{\Theta}(\epsilon^{-2}[\log(T/\delta)+d\log(1+L_0\sqrt{\lambda_2/\lambda_1}\epsilon^{-1})])$ in each iteration where $d=\max\{m,n\}$ is the dimension, $\alpha_p$ is the log-Sobolev coefficient of density $p$ and $\sigma(p)$ denotes $(\mathbb{E}_p[\|\theta\|^2])^{1/2}$.
\end{theorem}

Theorem \ref{main-text-outer-loop-thm} provides an estimate of the Max-Min gap. In the proof of Theorem \ref{main-text-outer-loop-thm}, we improve the commonly used two-step optimality condition in primal-dual analysis to a one-step optimality condition and one-step direct bounding. By setting proper $\gamma_t$, the convergence rate of Max-Min gap can be obtained. We can specify the hyper-parameters $\{\tau_t\},\{\eta_t\},\{\gamma_t\}$ and sub-problem error bound $\delta_{t,1},\delta_{t,2}$ for solving the minimax problem \eqref{eq:problem_particle}. 
% Our goal is to show that the Max-Min gap evaluated at the output solution
% \begin{align}
%     \Bar{w}_T=\frac{\sum_{t=1}^T\gamma_t w_t}{\sum_{t=1}^T\gamma_t},\notag
% \end{align}
% will converge to zero. In addition, we can prove a convergence guarantee about $w_T$ and $w_*$ in KL divergence along [Alogorithm Name]. 
Letting the input parameters be
\begin{equation}\label{parameter-setting}
\begin{split}
    &\mu_t = \mu=\frac{1}{2}\left(2+\lambda_2^2-\lambda_2\sqrt{4+\lambda_2^2}\right),\quad\eta_t=\tau_t=\frac{\lambda_2\mu}{1-\mu},\quad\gamma_t=\mu^{-t},
    \end{split}
\end{equation}
and defining $c(p)=\min\left\{\frac{1}{2}, \alpha_{p}, \frac{\alpha_{p}}{2(\sigma(p))^2}\right\}$, $c(q)=\min\left\{\frac{1}{2}, \alpha_{q}, \frac{\alpha_{q}}{2(\sigma(q))^2}\right\}$ as the upper bound of the inner loop errors $\delta_{t,1}$, $\delta_{t,2}$, we are ready to provide the following result for outer loop error bound of our algorithm with an inexact solver. Notice that $\mu$ in \eqref{parameter-setting} satisfies $\mu\leq1$ and $\mu^2-(2+\lambda_2^2)\mu+1=0$.
\begin{corollary}\label{main-text-outer-loop-complexity}
    Setting the parameters $\gamma_t,\, \eta_t,\, \tau_t,\, \mu_t$ as in Eq.~\eqref{parameter-setting} and assuming the sub-problem error bounds satisfy $\max\{\delta_{t,1},\delta_{t,2}\}\leq\frac{1}{2}\min\{c(p_t^*), c(q_t^*)\}T^{-2J}$ for any fixed positive integer $J$ and $\epsilon>0$ at each step-$t$, then the Max-Min gap between $\Bar{w}_T$ and $\bar{w}_T^*:=\arg\max_{w\in\mathcal{P}_2(\mathcal{X})\times\mathcal{P}_2(\mathcal{Y})}Q(\bar{w}_T,w)$ satisfies
    \begin{align}\label{Max-Min-gap}
        0\leq Q(\Bar{w}_T,\bar{w}_T^*)\leq&\frac{\lambda_2\mu^T}{1-\mu}\left[\mathrm{KL}(\bar{p}_T^*\|p_0)+\mathrm{KL}(\bar{q}_T^*\|q_0)\right]
        +8\epsilon+(10\lambda_1+\lambda_2+32)T^{-J}.
    \end{align}
    with probability at least $1-{\delta}$ for sample size $M=\Tilde{\Theta}(\epsilon^{-2}[\log(T/\delta)+d\log(1+L_0\sqrt{\lambda_2/\lambda_1}\epsilon^{-1})])$ in each iteration where $d=\max\{m,n\}$, $\Bar{w}_T=\frac{\sum_{t=1}^T\gamma_t w_t}{\sum_{t=1}^T\gamma_t}$. 
    % \begin{align}\label{KL-divergence}
    %     \frac{1}{2}\mathrm{KL}&(q_*\|q_T^*)+\mathrm{KL}(p_*\|p_T^*)\\
    %     &\leq\mu^{T-1}\left[\mathrm{KL}(q_*\|q_0^*)+\mathrm{KL}(p_*\|p_0^*)\right]+\frac{1}{(1-\mu)}[8\epsilon+(2\lambda_1+\lambda_2+16)T^{-J}]. \notag
    % \end{align}
\end{corollary}

% Corollary \ref{main-text-outer-loop-complexity} demonstrates that PAPAL achieves a pair of $\epsilon$ KL divergence accurate solution of the optimal distribution: $\max\{\text{KL}(q_*\|q), \text{KL}(p_*\|p)\}\leq \epsilon$ or a pair of $\epsilon$ Max-Min gap accurate solution of the optimal distribution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}\{Q(\Bar{w},w)\}\leq\epsilon$ after $\max\left\{\left(\frac{4}{(1-\mu)^2\epsilon}\right)^{1/J}, \frac{\log(4[\text{KL}(q_*\|q_0)+\text{KL}(p_*\|p_0)])-\log((1-\mu)\epsilon)}{\log(\mu^{-1})}\right\}$ iterations.

\noindent\textbf{Inner Loop Error Bound.}
We evaluate the complexity of ULA to obtain the global convergence. %In other words, we need to conclude the total complexity by taking both the outer loop and inner loop account.

% \begin{corollary}\label{main-text-cor-langevin-dynamic}
%        There exists a $t_0\in[0,1]$ such that $q_{t}(y)$ and $p_{t}(x)$ which denote the probability densities along Langevin dynamic \eqref{Langevin-dynamic-q} and \eqref{Langevin-dynamic-p} for time $t'$ with $t'-t_0\geq\Tilde{\Theta}(\frac{\log(C_0+1)+1}{\alpha})$ with objective $q_t^*(y)$ and $p_t^*(x)$. 
%        \begin{align}
%            dy_s=&-\nabla_y h^{(t)}(y_s)+dW_s^n,\label{Langevin-dynamic-q}
%            \\
%            dx_s=&-\nabla_x g^{(t)}(x_s)+dW_s^m.\label{Langevin-dynamic-p}
%        \end{align}\congfang{???}
%        The sub-problem error bounds satisfy the following evaluation: $\max\{\delta_{t,1}(p),\delta_{t,2}(p),\delta_{t,1}(q),\delta_{t,2}(q)\}\leq\max\{\mathrm{KL}(p_{t-1}\|p_t^*),\, \mathrm{KL}(q_{t-1}\|q_t^*),\, C_0\}e^{-\alpha(t'-t_0)}$ if Assumption \ref{ass:a1} holds. The constants $C_0, \alpha$ are depend on $\lambda_1, \lambda_2, \delta$\, (see Appendix \ref{Langevin-error} for details).
%         % \begin{align}
%         %     \max\left\{\left\|\frac{dp_{t}}{dp_t^*}-1\right\|_{\infty},\, \,  \left\|\frac{dq_{t}}{dq_t^*}-1\right\|_{\infty}\right\}\leq 
%         %     C_0(\lambda_1,\lambda_2,\delta)&e^{-\alpha(\lambda_1,\lambda_2,\delta)(t'-t_0)},\\
%         %     \max\{\mathrm{KL}(p_{t}\|p_t^*),\, \, \mathrm{KL}(q_{t}\|q_t^*)\}\leq e^{-\alpha(\lambda_1,\lambda_2,\delta)t'}\max\{\mathrm{KL}&(p_{t-1}\|p_t^*),\, \, \mathrm{KL}(q_{t-1}\|q_t^*)\}.
%         % \end{align}
%     \end{corollary}
\begin{theorem}\label{main-text-thm-ULA} \citep{vempala2019rapid}
    Assume that $f(\theta)$ is smooth and has $L_1$-Lipschitz gradient, and consider a probability density $p(\theta)\propto\exp{(-f(\theta))}$ satisfying the LSI with constant $\alpha$, ULA with step size $0<\iota<\frac{\alpha}{4L_1^2}$ satisfies $
        \mathrm{KL}(\rho_k||p)\leq e^{-\alpha\iota k}\mathrm{KL}(\rho_0||p)+\frac{8\iota d_\theta L_1^2}{\alpha}$
    where $d_\theta$ is the dimension.
\end{theorem}


\noindent\textbf{Global Convergence.} 
We can now conclude the global convergence of PAPAL using Corollary \ref{main-text-outer-loop-complexity} and Theorem \ref{main-text-thm-ULA}. The following part establishes the global error bound with obtaining a $\frac{1}{2}\min\{c(p_t^*), c(q_t^*)\}T^{-2J}$-accurate sub-problem solution at each step along ULA.
\begin{theorem}\label{main-text-global-convergence}
    Let $\epsilon$ be the desired accuracy. Under Assumptions \ref{ass:a1}, \ref{ass:a2} and \ref{ass:a4}, if we run Langevin algorithm with step size $\iota=\Theta\left(\min\left\{\frac{\lambda_1}{\lambda_2},\frac{\lambda_1^3}{\lambda_2^3}\right\}\frac{\lambda_2^2\epsilon^2}{(\max\{m,n\})^2(L_1+\lambda_1)^2\exp{(30/\lambda_2)}}\right)$ for $T_t=\tilde{\Theta}\left(\iota^{-1}\lambda_1^{-1}[\lambda_2\exp{(30/\lambda_2)}\right.$ $\left.\log(\epsilon^{-1})]\right)$ iterations on the inner loop, then we can achieve an $\epsilon$-mixed Nash equilibrium: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$ with probability at least $1-\delta$ when running Algorithm \ref{alg:algorithm} for iterations $T$
    and sample size $M$ with
    \begin{align*}
        &T=\Tilde{\Theta}\left(\max\left\{\log\left((\lambda_2+2)\epsilon^{-1}\right)/\log\left(\left(1-2\lambda_2/(\lambda_2+\sqrt{4+\lambda_2^2})\right)^{-1}\right),\, \, \epsilon^{-1/J}\right\}\right)\\
        &M = \Tilde{\Theta}\left(\epsilon^{-2}\left[\log\left(\frac{T}{{\delta}}\right)+d\log\left(1+L_0\sqrt{\frac{\lambda_2}{\lambda_1}}\epsilon^{-1}\right)\right]\right)
    \end{align*}
    on the outer loop, where $d = \max\{m,n\}$ is the dimension.
\end{theorem}
Then we obtain the computation time $T=\Tilde{\Theta}(\max\{\log(\epsilon^{-1})\lambda_2^{-1},\, \epsilon^{-1/J}\})$ if $\lambda_2 \rightarrow 0$, which indicates the limiting behavior of vanishing entropy regularizer. The dependence on $\lambda_2^{-1}$ in our convergence rate is a direct consequence of the classical LSI perturbation lemma \citep{holley1986logarithmic}, which is likely unavoidable for Langevin-based methods in the most general setting \citep{menzPoin2014}. Moreover, according to Eq.~\eqref{Max-Min-gap-control-entropy}, Theorem \ref{main-text-global-convergence} can also control $\mathrm{KL}(\Bar{p}\|\Bar{p}^*)$ and $\mathrm{KL}(\Bar{q}\|\Bar{q}^*)$ similarly.

% \begin{corollary}
%     Under Assumption \ref{ass:a1} and a fixed positive integer $J$, if we run the Langevin dynamic \eqref{Langevin-dynamic-q} and \eqref{Langevin-dynamic-p} with time $t'=\Tilde{\Theta}(\frac{J\log(T)}{\alpha})$ on the inner loop, and Algorithm \ref{alg:algorithm} for $T=\Tilde{\Theta}(\min\{\log(1/\epsilon), (1/\epsilon)^{1/J}\})$ iterations on the outer loop, then we can obtain an $\epsilon$-Max-Min-gap solution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$. Moreover, an $\epsilon$-KL-divergence-accurate solution: $\mathrm{KL}(q_*||q)+\mathrm{KL}(p_*||p)\leq\epsilon$ of objective \eqref{eq:problem_particle} can be achieved as well.
% \end{corollary}\congfang{theorem???}
% \begin{corollary}
%     Assume the parameter spaces of strategies $\cX$ and $\cY$ are compact Riemannian manifolds without boundary of dimension $m$, $n$ embedded in $\mathbb{R}^m$, $\mathbb{R}^n$ respectively and Assumptions \ref{ass:a1}, \ref{ass:a2} and \ref{ass:a3} hold. We can obtain an $\epsilon$-Max-Min-gap solution: $\max_{w\in\cP_2(\cX)\times\cP_2(\cY)}Q(\Bar{w},w)\leq\epsilon$ and an $\epsilon$-KL-divergence-accurate solution: $\mathrm{KL}(q_*||q)+\mathrm{KL}(p_*||p)\leq\epsilon$ of objective \eqref{eq:problem_particle} with running Algorithm \ref{alg:algorithm} for $T=\Tilde{\Theta}(\min\{\log(1/\epsilon), (1/\epsilon)^{1/J}\})$ iterations on the outer loop, and the ULA with step size $\sigma_t=\Theta\left(\min\left\{c_0\min\{\alpha, c_1\}, \frac{1}{\hat{C}_1^2\hat{C}_0^2}T^{-2J}\right\}\right)$ for $T_t=\Tilde{\Theta}\left(\frac{2J\log(T)}{\alpha\sigma_t}\right)$ on the inner loop where $J$ is a fixed positive integer.
% \end{corollary}
% Th\epsilondefinitions of $\nabla_x h^{(t)}(x)$ and $\nabla_y g^{(t)}(y)$ in Algorithm \ref{alg:algorithm} satisfy
% \begin{align}
%     \nabla_yh^{(t)}(y)=&\sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)\frac{1}{\lambda_2+\tau_i}\left\{\mu_{i}\right.
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \mathbb{E}_{\tilde{X}^{(i-2)}}[\nabla_y f(\cdot,y)]-(1+\mu_i)
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \left.\mathbb{E}_{\tilde{X}^{(i-1)}}[\nabla_y f(\cdot, y)]\right\}+(2+\delta)
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \,  \sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)\frac{1}{\lambda_2+\tau_i}\|y\|^\delta y
%     \notag
%     \\
%     &\, \, \, \, +\frac{2\lambda_1}{\lambda_2}\left(\prod_{l=1}^t\frac{\tau_l}{\lambda_2+\tau_l}\right)y,
%     \notag
%     \\
%     \nabla_x g^{(t)}(x)=&\sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)\frac{1}{\lambda_2+\eta_i}
%     \notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \, \mathbb{E}_{\tilde{Y}^{(i)}}[\nabla_x f(x,\cdot)]+(2+\delta)\notag
%     \\
%     &\, \, \, \, \, \, \, \, \, \, \, \sum_{i=1}^t\left(\prod_{l=i+1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)\frac{1}{\lambda_2+\eta_i}\|x\|^\delta x
%     \notag
%     \\
%     &\, \, \, \, +\frac{2\lambda_1}{\lambda_2}\left(\prod_{l=1}^t\frac{\eta_l}{\lambda_2+\eta_l}\right)x.\notag
% \end{align}
